First Align, then Predict: Understanding the Cross-Lingual Ability of Multilingual BERT

Multilingual pretrained language models have demonstrated remarkable zero-shot cross-lingual transfer capabilities. Such transfer emerges by fine-tuning on a task of interest in one language and evaluating on a distinct language, not seen during the fine-tuning. Despite promising results, we still lack a proper understanding of the source of this transfer. Using a novel layer ablation technique and analyses of the model's internal representations, we show that multilingual BERT, a popular multilingual language model, can be viewed as the stacking of two sub-networks: a multilingual encoder followed by a task-specific language-agnostic predictor. While the encoder is crucial for cross-lingual transfer and remains mostly unchanged during fine-tuning, the task predictor has little importance on the transfer and can be reinitialized during fine-tuning. We present extensive experiments with three distinct tasks, seventeen typologically diverse languages and multiple domains to support our hypothesis.

==> Makefile <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = eacl-2021-camera-ready
# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles = 



#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	pdflatex  $(latexfile).tex 

pdf :	$(latexfile).pdf 

bib : $(latexfile).tex
	pdflatex $(latexfile)
	bibtex $(latexfile)
	pdflatex $(latexfile)
	pdflatex $(latexfile)
	bibtex $(latexfile)
	pdflatex $(latexfile)
	pdflatex $(latexfile) 

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
check:
	cat $(latexfile).log | grep undef

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

view: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf


gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex &


up:
	svn up ./
	
commit:
#	svn add ./
	svn commit -m "Modif2" ./
	
	
ebib:
	open emnlp2014.bib
	

==> re_init_table_with_x3.tex <==




\begin{table*}[t!]
\footnotesize\centering
\scalebox{0.85}{ % was .7775
\begin{tabular}{llrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     &&  \multicolumn{4}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     Setting&Eval&\textsc{\standardFineTune} & \Delta~\textsc{All} &  \Delta~\textsc{0-3} & \Delta~\textsc{4-7} & \Delta~\textsc{8-11} &
     %\textit{Re-Init.} & \textsc{None } & \textsc{0} & \textsc{1} & \textsc{2} & \textsc{5} & \textsc{8} & \textsc{10} & \textsc{11} & \textsc{0-1} & \textsc{1-2} & \textsc{2-3} & \textsc{4-5} & \textsc{6-7} & \textsc{8-9} & \textsc{10-11} & \textsc{0-2} & \textsc{1-3} & \textsc{4-6} & \textsc{9-11}  \\%& \\
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    \midrule

&&  \multicolumn{9}{c}{\textit{Parsing}} \\
  \inlang & \textsc{English} & 88.62 & \cellcolor{pink}-14.04 & %\cellcolor{lightgreen}-0.85 & \cellcolor{lightgreen}-0.52 & \cellcolor{lightgreen}-1.37 & \cellcolor{lightgreen}-1.83 &
  \cellcolor{pink}-5.51 & \cellcolor{lightgreen}-3.24 & \cellcolor{mediumspringgreen}0.07 \\ 
\hdashline
 \crosslang& \textsc{French} & 68.86 & \cellcolor{brightlavender}-65.16 & 
 %\cellcolor{lightgreen}-3.14 & \cellcolor{lightgreen}-3.65 & \cellcolor{brightlavender}-13.55 & \cellcolor{pink}-7.55 & 
 \cellcolor{brightlavender}-31.58 & \cellcolor{pink}-7.04 & \cellcolor{mediumspringgreen}0.40 \\ 
 & \textsc{German} & 67.53 & %\cellcolor{brightlavender}-62.80 & \cellcolor{lightgreen}-2.55 & \cellcolor{lightgreen}-2.33 & %\cellcolor{brightlavender}-10.44 & 
 \cellcolor{pink}-6.91 & \cellcolor{brightlavender}-31.47 & \cellcolor{pink}-8.15 & \cellcolor{lightgreen}-0.32 \\ 
 
 & \textsc{Turkish} & 28.37 & \cellcolor{brightlavender}-25.61 & 
 %\cellcolor{pink}-6.71 & \cellcolor{lightgreen}-4.60 & \cellcolor{brightlavender}-11.58 & \cellcolor{pink}-7.16 & 
 \cellcolor{brightlavender}-18.67 & \cellcolor{pink}-7.43 & \cellcolor{mediumspringgreen}0.97 \\ 
 & \textsc{Indonesian} & 45.19 & \cellcolor{brightlavender}-40.20 & %\cellcolor{lightgreen}-1.86 & \cellcolor{lightgreen}-1.71 & \cellcolor{pink}-5.36 & \cellcolor{pink}-6.10 & 
 \cellcolor{brightlavender}-14.84 & \cellcolor{lightgreen}-4.34 & \cellcolor{mediumspringgreen}2.34 \\ 
 & \textsc{Russian} & 59.57 & \cellcolor{brightlavender}-56.63 & %\cellcolor{lightgreen}-1.76 & \cellcolor{lightgreen}-2.04 & \cellcolor{pink}-5.47 & \cellcolor{pink}-6.06 & 
 \cellcolor{brightlavender}-20.99 & \cellcolor{pink}-7.17 & \cellcolor{mediumspringgreen}1.15 \\ 
 & \textsc{Arabic} & 23.51 & \cellcolor{brightlavender}-20.32 & %\cellcolor{mediumspringgreen}0.15 & \cellcolor{lightgreen}-0.02 & \cellcolor{lightgreen}-2.50 & \cellcolor{lightgreen}-3.95 & 
 \cellcolor{brightlavender}-10.25 & \cellcolor{pink}-5.24 & \cellcolor{mediumspringgreen}0.42 \\ 
 \hdashline
Summary & \gap  & -39.78 & \cellcolor{brightlavender}-70.86 & %\cellcolor{lightgreen}-41.57 & %\cellcolor{lightgreen}-41.65 & 
%\cellcolor{pink}-46.56 & \cellcolor{pink}-44.24 & 
\cellcolor{brightlavender}-55.56 & \cellcolor{pink}-43.10 & \cellcolor{green}-39.02 \\ 
\midrule

&&  \multicolumn{9}{c}{\textit{POS}} \\

 \inlang& \textsc{English} & 96.47 & \cellcolor{pink}-8.76 & %\cellcolor{lightgreen}-0.39 & \cellcolor{lightgreen}-0.23 & \cellcolor{lightgreen}-0.53 & \cellcolor{lightgreen}-0.75 & 
 \cellcolor{lightgreen}-2.42 & \cellcolor{lightgreen}-1.02 & \cellcolor{mediumspringgreen}0.04 \\ 
 
 \hdashline
 
\crosslang & \textsc{French} & 88.23 & \cellcolor{brightlavender}-59.28 & 
 %\cellcolor{lightgreen}-1.53 & \cellcolor{lightgreen}-0.57 & \cellcolor{pink}-8.39 & \cellcolor{lightgreen}-1.09 & 
 \cellcolor{brightlavender}-25.96 & \cellcolor{lightgreen}-1.86 & \cellcolor{mediumspringgreen}0.03 \\ 
 
 & \textsc{German} & 90.51 & \cellcolor{brightlavender}-61.59 & %\cellcolor{lightgreen}-2.25 & \cellcolor{lightgreen}-0.98 & \cellcolor{pink}-8.25 & \cellcolor{lightgreen}-2.13 & 
 \cellcolor{brightlavender}-31.35 & \cellcolor{lightgreen}-1.39 & \cellcolor{mediumspringgreen}0.13 \\ 
 & \textsc{Turkish} & 72.49 & \cellcolor{brightlavender}-40.26 & %\cellcolor{brightlavender}-10.32 & %\cellcolor{pink}-6.32 & \cellcolor{brightlavender}-17.99 & \cellcolor{pink}-9.27 & 
 \cellcolor{brightlavender}-28.33 & \cellcolor{lightgreen}-3.19 & \cellcolor{mediumspringgreen}0.59 \\ 
 
 & \textsc{Indonesian} & 84.02 & \cellcolor{brightlavender}-47.04 & %\cellcolor{lightgreen}-1.86 & \cellcolor{lightgreen}-1.12 & \cellcolor{lightgreen}-3.88 & \cellcolor{lightgreen}-2.61 & 
 \cellcolor{brightlavender}-11.60 & \cellcolor{lightgreen}-1.43 & \cellcolor{mediumspringgreen}0.07 \\ 
 & \textsc{Russian} & 83.04 & \cellcolor{brightlavender}-50.41 & %\cellcolor{mediumspringgreen}0.10 & \cellcolor{mediumspringgreen}0.59 & \cellcolor{lightgreen}-1.09 & \cellcolor{lightgreen}-0.78 & 
 \cellcolor{brightlavender}-12.71 & \cellcolor{lightgreen}-0.48 & \cellcolor{mediumspringgreen}0.15 \\ 
 
 & \textsc{Arabic} & 56.44 & \cellcolor{brightlavender}-36.83 & %\cellcolor{mediumspringgreen}1.66 & \cellcolor{mediumspringgreen}1.62 & \cellcolor{mediumspringgreen}1.45 & \cellcolor{lightgreen}-0.82 & 
 \cellcolor{lightgreen}-4.17 & \cellcolor{lightgreen}-2.84 & \cellcolor{mediumspringgreen}2.39 \\ 
Summary & \textsc{CL Transfer Gap}  & -17.35 & \cellcolor{brightlavender}-57.82 & 
%-19.32 & -18.25 & -23.18 & -19.38 &
\cellcolor{lightgreen}-33.95 & \cellcolor{lightgreen}-18.19 & \cellcolor{mediumspringgreen}-16.83 \\ 
\midrule

&&  \multicolumn{9}{c}{\textit{NER}} \\
 \inlang & \textsc{English} & 82.98 & \cellcolor{brightlavender}-26.42 & 
 %\cellcolor{lightgreen}-1.52 & \cellcolor{lightgreen}-0.98 & \cellcolor{lightgreen}-3.35 & \cellcolor{lightgreen}-3.73 & 
 \cellcolor{pink}-13.90 & \cellcolor{lightgreen}-3.08 & \cellcolor{lightgreen}-0.71 \\ 

\hdashline
 \crosslang& \textsc{French} & 76.65 & \cellcolor{brightlavender}-41.30 & 
 %\cellcolor{lightgreen}-1.19 & \cellcolor{mediumspringgreen}0.92 & \cellcolor{pink}-6.71 & \cellcolor{lightgreen}-3.82 & 
 \cellcolor{brightlavender}-20.86 & \cellcolor{lightgreen}-3.53 & \cellcolor{lightgreen}-0.88 \\ 
 
 & \textsc{German} & 76.35 & \cellcolor{brightlavender}-57.39 & %\cellcolor{lightgreen}-2.62 & \cellcolor{lightgreen}-0.96 & \cellcolor{brightlavender}-10.17 & \cellcolor{pink}-6.23 & 
 \cellcolor{brightlavender}-33.98 & \cellcolor{pink}-5.20 & \cellcolor{lightgreen}-0.85 \\ 
 
 & \textsc{Turkish} & 67.45 & \cellcolor{brightlavender}-46.69 & %\cellcolor{lightgreen}-4.91 & \cellcolor{lightgreen}-2.61 & \cellcolor{brightlavender}-15.25 & \cellcolor{brightlavender}-10.34 & 
 \cellcolor{brightlavender}-28.07 & \cellcolor{pink}-6.01 & \cellcolor{lightgreen}-0.83 \\ 
 
 & \textsc{Indonesian} & 54.10 & \cellcolor{brightlavender}-32.90 & %\cellcolor{lightgreen}-4.91 & \cellcolor{lightgreen}-4.83 & \cellcolor{pink}-7.60 & \cellcolor{pink}-7.23 & 
 \cellcolor{brightlavender}-17.99 & \cellcolor{pink}-8.04 & \cellcolor{pink}-5.87 \\ 
 
 & \textsc{Russian} & 58.28 & \cellcolor{brightlavender}-50.84 & %\cellcolor{lightgreen}-2.65 & \cellcolor{lightgreen}-0.20 & \cellcolor{pink}-7.61 & \cellcolor{pink}-5.39 & 
 \cellcolor{brightlavender}-23.62 & \cellcolor{pink}-6.25 & \cellcolor{mediumspringgreen}0.84 \\ 
 & \textsc{Arabic} & 41.88 & \cellcolor{brightlavender}-36.40 & %\cellcolor{pink}-6.09 & \cellcolor{pink}-7.08 & \cellcolor{pink}-9.51 & \cellcolor{pink}-9.57 & 
 \cellcolor{brightlavender}-20.03 & \cellcolor{lightgreen}-3.21 & \cellcolor{lightgreen}-0.65 \\ 
\hdashline 
Summary & \gap  & -20.53 & \cellcolor{brightlavender}-38.37 & %\cellcolor{lightgreen}-22.74 & \cellcolor{lightgreen}-22.01 & \cellcolor{pink}-26.65 & \cellcolor{pink}-23.89 & 
\cellcolor{brightlavender}-30.72 & \cellcolor{lightgreen}-22.83 & \cellcolor{lightgreen}-21.20 
\\
\bottomrule

\end{tabular}
}
\caption{Relative Zero shot Cross-Lingual performance compared to reference (\textsc{Ref} column) when fine-tuning the model applying  \reinit (section \ref{sec:controlled_exp}) to specific set of layers. Source language is English. Bottom-line model \textsc{ALL} (for all layers randomly initialized) corresponds to a model trained from scratch on the task.
\textsc{Ref} column is the \standardFineTune fine-tuned model. 
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Std min/median/max,Parsing:0.02/0.34/1.48,POS:0.01/0.5/2.38 ,NER:0.0/0.47/2.62
%\colorbox{blue}{xxx}
\colorbox{mediumspringgreen}{$\geq$ reference}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
\colorbox{lightgreen}{$\leq$ reference}
\colorbox{pink}{$\geq$ 5 points drop}
\colorbox{brightlavender}{$\geq$ 15 points drop} 
%\textcolor{brightlavender}{$\leq$ 20 points drop}}
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
}
\label{tab:re_init_x4_all_reduce}%re_init_x4_all_reduce}
\end{table*}

==> tables/domain_01.tex <==




\begin{table*}[t!]
\footnotesize\centering
\scalebox{1.0}{ % was .7775
\begin{tabular}{lrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
      Evaluation Language \& Domain &\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}} \\%\testsc{Ref} & \textsc{0-1} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
\midrule
&\underline{Ref}&\underline{0-1}&\underline{Ref}&\underline{0-1}&\underline{Ref}&\underline{0-1}\\
%\multicolumn{4}{c}{\textit{\inlang}}&&&&\\

%\textsc{In} & \textsc{In} & \textsc{In} & en & 86.00 & \cellcolor{lightgreen}-0.42 \\ 

\multicolumn{1}{c}{\textit{\inlang \& \textit{\indomain}}}&&\\

\textsc{English test set} & 86.00 & \cellcolor{lightgreen}-0.42 & 95.60 & \cellcolor{lightgreen}-0.64 & 83.17& \cellcolor{lightgreen}1.81\\  
\hdashline

\multicolumn{1}{c}{\textit{\inlang  \& \textit{Out-of-Domain}}}&&\\
\textsc{English Literature} & 76.65 & \cellcolor{lightgreen}-0.93 & 93.28 & \cellcolor{lightgreen}-0.60 &-&-\\ 
\textsc{English  Web Media} & 73.76 & \cellcolor{lightgreen}-1.26 & 89.87 & \cellcolor{lightgreen}-1.06 &-&-\\ 
\textsc{English  Noisy Tweets} & 44.75 & \cellcolor{lightgreen}-1.22 & 69.68  & \cellcolor{lightgreen}-1.82 &-&-\\
\textsc{English  News} & - &-& - & - & 58.22& \cellcolor{lightgreen}-1.51 \\ 

\hdashline

\multicolumn{1}{c}{\crosslang \& \textit{In-Domain}}&&&&\\

\textsc{French Translation Test Set} & 80.56 & \cellcolor{pink}-4.49 & 93.30& \cellcolor{pink}-2.79&-&-\\

\textsc{French \indomain} & 68.23 & \cellcolor{red}-5.21 & 90.53 & \cellcolor{pink}-3.64 & 78.57 & \cellcolor{pink}-2.93
\\
\hdashline
\multicolumn{1}{c}{\crosslang \& \textit{Out-of-Domain}}&&\\
\textsc{French Speech} & 53.97 & \cellcolor{red}-6.31 & 83.67 & \cellcolor{red}-9.11 &-&- \\ 




%\midrule
%&\multicolumn{2}{c}{\textit{POS}}\\

%\textsc{English} & 95.60 & \cellcolor{lightgreen}-0.64 \\ 
%\hdashline
%\multicolumn{1}{c}{\inlang \textit{Out-of-Domain}}&&\\

%\textsc{English Litterature} & 
%93.28 & \cellcolor{lightgreen}-0.60 \\ 
%\textsc{Web} & 
%89.87 & \cellcolor{lightgreen}-1.06 \\ 
%\textsc{English UGC} & 69.68 & \cellcolor{lightgreen}-2.00 \\ 

%\hdashline
%\multicolumn{1}{c}{\crosslang \textit{In-Domain}}&&\\

%\textsc{Translate} & 93.30 & \cellcolor{pink}-2.79 \\ 
%\textsc{French} & 90.53 & \cellcolor{pink}-3.64 \\ 
%\hdashline
%\multicolumn{1}{c}{\crosslang \textit{Out-of-Domain}}&&\\

%\textsc{French Speech} & 83.67 & \cellcolor{red}-9.11 \\ 



\bottomrule

\end{tabular}
}

\caption{Domain analysis: 
Relative Zero shot Cross-Lingual performance compared to reference (\textsc{Ref} column) when fine-tuning the model applying  \reinit (section \ref{sec:controlled_exp}) to  layer 0 to 3. Source language is English. 
Reference column is \standardFineTune fine-tuned model. Reporting 4 different settings as a combination of \{\indomain,\textit{Out-of-Domain}\} and \{\inlang,cross-lingual\} focusing on English vs. French.
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
}
\label{tab:domain_appendix}
\end{table*}

==> tables/domain_analysis_old.tex <==



\begin{table}[ht!]
\footnotesize\centering
\scalebox{0.88}{ % was .7775
\begin{tabular}{llrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     %\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
       %Language \& Domain
      \textit{Setting}&\textit{Evaluation}&\textsc{Ref}&\Delta\textsc{0-3}& %\testsc{Ref} & \textsc{0-1} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
%\midrule
%&\underline{Ref}&\underline{0-1}\\
%\multicolumn{4}{c}{\textit{\inlang}}&&&&\\

%\textsc{In} & \textsc{In} & \textsc{In} & en & 86.00 & \cellcolor{lightgreen}-0.42 \\ 
%\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\

&& \multicolumn{2}{c}{\textit{Parsing}}&
\textit{English \& In-Dist}&\textsc{Test split} & 86.00 & \cellcolor{lightgreen}-6.23\\
\hdashline
\textit{English~\&~OOD} &\textsc{Literature} & 76.65 & \cellcolor{lightgreen}-5.93 \\  
&\textsc{Web Media} & 73.76 & \cellcolor{lightgreen}-6.93\\  
&\textsc{Noisy UGC} & 44.75 & \cellcolor{lightgreen}-7.22\\%\\ 

\hdashline
\textit{French \& In-Domain} &\textsc{Translation} & 80.56 & \cellcolor{brightlavender}-33.32& 
&\textsc{Wiki \& News} & 68.23 & \cellcolor{brightlavender}-30.59\\

\midrule
&& \multicolumn{2}{c}{\textit{POS}}&

\textit{English \& In-Dist}&\textsc{Test split}  &  96.44&\cellcolor{lightgreen}-2.67\\%\\83.17 & \cellcolor{pink}-14.81 \\
\hdashline

\textit{English \& OOD}&\textsc{Literature} &93.28 & \cellcolor{lightgreen}-4.64 \\  
&\textsc{Web Media} & 90.11 & \cellcolor{lightgreen}-4.27&
&\textsc{Noisy UGC} & 69.60  & \cellcolor{lightgreen}-7.12 \\%\\ 

\hdashline
\textit{French \& In-Domain}&\textsc{Translation} & 93.27 & \cellcolor{brightlavender}-28.11\\
&\textsc{Wiki \& News} &90.89 & \cellcolor{brightlavender}-29.33\\

\midrule
&& \multicolumn{2}{c}{\textit{NER}}&

\textit{English \& In-Dist}&\textsc{Test split} & 83.17 & \cellcolor{pink}-14.81 \\
\hdashline
\textit{English \& OOD} &\textsc{News} & 56.80 & \cellcolor{pink}-11.22\\

\hdashline
\textit{French \& In-Domain}&\textsc{Wiki} & 78.57 & \cellcolor{brightlavender}-41.46\\



%\textsc{\indomain} & 68.23 & \cellcolor{brightlavender}-30.59&90.89 & \cellcolor{brightlavender}-29.33& 78.57 & \cellcolor{brightlavender}-41.46\\
%\hdashline
%\multicolumn{1}{c}{ %-\textit{Out-of-Domain}}&\\
%\textsc{\outdomain} & 53.97 & \cellcolor{brightlavender}-24.31 & 90.89 & \cellcolor{brightlavender}-29.33&-&-\\



\bottomrule

\end{tabular}
}

\caption{Zero shot Cross-Lingual performance compared to \standardFineTune (\textsc{Ref}) when applying  \reinit to  layer 0 to 3. %Source language is English. 
%Reference column is model fine-tuned when no \reinit is applied. Reporting 4 different settings as a combination of \{\indomain,\outdomain\} and \{\inlang,\crosslang\} focusing on English vs. French. Trans. Test is the French translation of the Test split.
Details on test data can be found in Appendix~\ref{sec:domain_dataset_details}.
%\colorbox{mediumspringgreen}{$\geq$ reference}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
%\colorbox{lightgreen}{$\geq$ reference}
\colorbox{lightgreen}{$\geq$ 10 points drop}
\colorbox{pink}{$\leq$ 15 points drop}
\colorbox{brightlavender}{$\geq$ 15 points drop} 
%POS tagging and aboslute performance can be found in Appendix.
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
}
\label{tab:domain}
\end{table}


==> tables/domain_gap.tex <==



\begin{table}[ht!]
\footnotesize\centering
\scalebox{0.88}{ % was .7775
\begin{tabular}{llrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     %\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
       %Language \& Domain
       &&&\multicolumn{2}{c}{\textit{\underline{\textit{Random-init of..}}}}\\ %\testsc{Ref} &
      Setting&Evaluation&\textsc{Ref}&\textsc{0-2}&\textsc{9-11}& %\testsc{Ref} & \textsc{0-1} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
%\midrule
%&\underline{Ref}&\underline{0-1}\\
%\multicolumn{4}{c}{\textit{\inlang}}&&&&\\

%\textsc{In} & \textsc{In} & \textsc{In} & en & 86.00 & \cellcolor{lightgreen}-0.42 \\ 
%\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
&& \multicolumn{3}{c}{\textit{Parsing}}&
  \textit{\textit{same-lang} perf.} & \textsc{English}  & \textit{86.60} & \textit{82.26} & \textit{88.35} \\ 
 \hdashline
 \textit{domain gap} & \textsc{Litterature} & 9.90 & \cellcolor{mediumspringgreen}9.39 & \cellcolor{lightgreen}10.85 \\ 
 & \textsc{Web} & 12.77 & \cellcolor{lightgreen}13.34 & \cellcolor{lightgreen}13.68 \\ 
 & \textsc{Tweets} & 41.66 & \cellcolor{lightgreen}42.73 & \cellcolor{lightgreen}41.88 \\ 
 \hdashline
  \gap & \textsc{Translate} & 5.95 & \cellcolor{brightlavender}18.49 & \cellcolor{mediumspringgreen}5.88 \\ 
 
 & \textsc{\indomain} & 18.44 & \cellcolor{brightlavender}30.74 & \cellcolor{mediumspringgreen}17.84 \\ 
 \midrule
 
 
 
 
&& \multicolumn{3}{c}{\textit{POS}}&

 \textit{\textit{same-lang} perf.} & \textsc{English} & \textit{95.84} & \textit{94.23} & \textit{95.88} \\ 
 \hdashline
 \textit{domain gap} & \textsc{Litterature} & 2.58 & \cellcolor{lightgreen}3.21 & \cellcolor{lightgreen}2.64 \\ 
 & \textsc{Web} & 5.81 & \cellcolor{lightgreen}6.89 & \cellcolor{lightgreen}5.92 \\ 
 & \textsc{Tweets} & 26.84 & \cellcolor{lightgreen}29.56 & \cellcolor{mediumspringgreen}26.21 \\ 
 \hdashline
 \gap  & \textsc{Translate} & 2.29 & \cellcolor{pink}10.76 & \cellcolor{mediumspringgreen}2.11 \\ 
 & \textsc{\indomain} & 4.79 & \cellcolor{pink}14.26 & \cellcolor{mediumspringgreen}4.34 \\ 
 \midrule
 && \multicolumn{3}{c}{\textit{NER}}&
  \textit{\textit{same-lang} perf.} & \textsc{English} & \textit{82.99} & \textit{76.73} & \textit{82.24} \\ 
  \hdashline
  \textit{domain gap}& \textsc{News} & 26.96 & \cellcolor{lightgreen}28.64 & \cellcolor{mediumspringgreen}23.69 \\
  \hdashline
 \gap& \textsc{French} & 6.30 & \cellcolor{pink}11.54& \cellcolor{mediumspringgreen}6.12 \\ 
 

%Summary & \textsc{ Average }  & 9.13 & 14.45 & 8.83 \\ 
%\textsc{\indomain} & 68.23 & \cellcolor{brightlavender}-30.59&90.89 & \cellcolor{brightlavender}-29.33& 78.57 & \cellcolor{brightlavender}-41.46\\
%\hdashline
%\multicolumn{1}{c}{ %-\textit{Out-of-Domain}}&\\
%\textsc{\outdomain} & 53.97 & \cellcolor{brightlavender}-24.31 & 90.89 & \cellcolor{brightlavender}-29.33&-&-\\



\bottomrule

\end{tabular}
}

\caption{Zero-shot \gap  when applying  \reinit on several \outdomain English sets in comparison with \crosslang evaluation (\textsc{Ref} is the \standardFineTune model). %Source language is English. 
%Reference column is model fine-tuned when no \reinit is applied. Reporting 4 different settings as a combination of \{\indomain,\outdomain\} and \{\inlang,\crosslang\} focusing on English vs. French. Trans. Test is the French translation of the Test split.
Details on test data can be found in Appendix~\ref{sec:domain_dataset_details}.
%\colorbox{mediumspringgreen}{$\geq$ reference}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
%\colorbox{lightgreen}{$\geq$ reference}
\colorbox{mediumspringgreen}{$\leq$ \textsc{Ref}}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
\colorbox{lightgreen}{$>$  \textsc{Ref}}
\colorbox{pink}{$\geq$ +5 points}
\colorbox{brightlavender}{$\geq$ +10 points }
%POS tagging and aboslute performance can be found in Appendix.
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
}
\label{tab:domain}
\end{table}


==> tables/domain_table.tex <==



\begin{table}[ht!]
\footnotesize\centering
\scalebox{0.81}{ % was .7775
\begin{tabular}{lrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     \textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
\multicolumn{1}{c}{\textbf{English}}&&\\
       %Language \& Domain
      &\underline{Ref}&\Delta~\underline{0-3}&\underline{Ref}&\underline{0-3}&\underline{Ref}&\underline{0-3} \\%\testsc{Ref} & \textsc{0-1} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
%\midrule
%&\underline{Ref}&\underline{0-1}\\
%\multicolumn{4}{c}{\textit{\inlang}}&&&&\\

%\textsc{In} & \textsc{In} & \textsc{In} & en & 86.00 & \cellcolor{lightgreen}-0.42 \\ 


\textsc{Test split} & 86.00 & \cellcolor{lightgreen}-6.23 &  96.44 & \cellcolor{lightgreen}-2.67 &  83.17 & \cellcolor{pink}-14.81 \\
\hdashline

%\multicolumn{1}{c}{\textit{\inlang  \& \textit{Out-of-Domain}}}&\\
\multicolumn{1}{c}{\textit{ \textit{Out-of-Domain}}}&\\
\textsc{New} & - &  - & - & - & 56.8 & \cellcolor{pink}-11.22\\
\textsc{Literature} & 76.65 & \cellcolor{lightgreen}-5.93&93.28 & \cellcolor{lightgreen}-4.64 &-&-\\  
\textsc{Web Media} & 73.76 & \cellcolor{lightgreen}-6.93&90.11 & \cellcolor{lightgreen}-4.27&-&-\\  
\textsc{Noisy UGC} & 44.75 & \cellcolor{lightgreen}-7.22&69.60  & \cellcolor{lightgreen}-7.12&-&-\\%\\ \textsc{English  News} & - &-& - & - & 58.22& \cellcolor{lightgreen}-1.51 \\ 

\hdashline

\multicolumn{1}{c}{\textbf{French}}&\\

\textsc{Translation Test} & 80.56 & \cellcolor{brightlavender}-33.32& 93.27 & \cellcolor{brightlavender}-28.11&-&-\\

\textsc{\indomain} & 68.23 & \cellcolor{brightlavender}-30.59&90.89 & \cellcolor{brightlavender}-29.33& 78.57 & \cellcolor{brightlavender}-41.46\\
%\hdashline
%\multicolumn{1}{c}{ %-\textit{Out-of-Domain}}&\\
\textsc{\outdomain} & 53.97 & \cellcolor{brightlavender}-24.31 & 90.89 & \cellcolor{brightlavender}-29.33&-&-\\



\bottomrule

\end{tabular}
}

\caption{Domain analysis: 
Relative Zero shot Cross-Lingual performance compared to reference (\textsc{Ref} column) when fine-tuning the model applying  \reinit (section \ref{sec:controlled_exp}) to  layer 0 to 3. Source language is English. 
Reference column is model fine-tuned when no \reinit is applied. Reporting 4 different settings as a combination of \{\indomain,\outdomain\} and \{\inlang,\crosslang\} focusing on English vs. French. Trans. Test is the French translation of the Test split.
More details on evaluation data can be found in Appendix~\ref{sec:domain_dataset_details}.
%\colorbox{mediumspringgreen}{$\geq$ reference}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
%\colorbox{lightgreen}{$\geq$ reference}
\colorbox{lightgreen}{$\geq$ 10 points drop}
\colorbox{pink}{$\leq$ 15 points drop}
\colorbox{brightlavender}{$\leq$ 15 points drop} 
%POS tagging and aboslute performance can be found in Appendix.
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
}
\label{tab:domain}
\end{table}


==> tables/freeze_x_reinit.tex <==


\begin{table}[t!]
\footnotesize\centering
\scalebox{0.9}{ % was .7775
\begin{tabular}{lrrrr}
    \toprule
    %Scenario  & 
    ~~~~~~\textit{Decoder} & \multicolumn{2}{c}{\textsc{Pretrained}} &  \multicolumn{2}{c}{\reinit} & 
    \textit{Model} & \textsc{In-Lang} &  \textsc{X-Gap} & \textsc{In-Lang} &  \textsc{X-Gap} & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     %\textit{Fine-tuning} & \textsc{Standart} & \textsc{Attention only} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
&\multicolumn{4}{c}{\textit{Parsing}}\\


\standardFineTune & 88.62  & -39.74 &-& - \\

\hdashline
\multicolumn{1}{c}{\textit{Fine-tuning all}}&\\
%\testsc{Tune Bottom-5}  & \textit{run} &\textit{run}  & 87.25 & 40.65  \\
\testsc{Tune Bottom-1}  & 88.62 &-39.74 &  79.97 & -48.80\\

\testsc{Tune Bottom-3}  & 88.62 &-39.74 & 84.89 & -43.99 \\

\testsc{Tune Bottom-5}  & 88.62 &-39.74 & 87.25 & -40.65  \\
\testsc{Tune Bottom-8}  & 88.62 & -39.74 & 89.96 & -37.55  \\
\testsc{Tune Bottom-10}  & 88.62 & -39.74 & 88.60  & -39.70  \\
%\testsc{Tune Bottom-6}  & run & run &  &   \\
%\testsc{Tune Bottom-8}  & 88.46 & 39.01 & 89.96 & 37.55  \\
%\testsc{Tune Bottom-10}  & 88.81 & 39.72 & 88.60  & 39.70  \\
\hdashline
\multicolumn{1}{c}{\textit{Freezing encoder}}&\\
\testsc{Freeze Bottom-1}  &88.65 &-39.05& 77.23& -45.64\\
\testsc{Freeze Bottom-3}  & 88.33 & -39.34 & 81.80 & -41.06\\
\testsc{Freeze Bottom-5}  &\textit{run} & \textit{run}& 83.87 & -38.07 \\
\testsc{Freeze Bottom-6}  &\textit{run} & \textit{run}& 83.86 & -37.70 \\ %-10608554 - 10626355
\testsc{Freeze Bottom-8}  & 84.27 & -41.21 & 82.45  & 37.55 \\%-%-10608554 - 10626355
\testsc{Freeze Bottom-10} & 76.24 & -41.27  & 77.18 & -37.26\\%-10608554 - 10626355

%\hdashline
%\multicolumn{1}{c}{\textit{\reinit Decoder}}&\\
%\testsc{Encoder-6 + Decode-R}  & & & \\
%\testsc{Encoder-7 + Decode-R}  &&& 83.86  & 37.70 \\
%\testsc{Encoder-9 + Decode-R}  &&& 82.45  & 37.55 \\

%\textsc{English} & 87.04 & 79.18 \\ \textsc{\crosslang Gap} & -40.62 & -57.83 \\ 
% reporting result ~ bottom-3 instead of bottom-5
\midrule
&\multicolumn{4}{c}{\textit{POS}}\\


\standardFineTune & 96.43 & -17.38 &-&-  \\

\hdashline
\multicolumn{1}{c}{\textit{Fine-tuning all}}&\\
\testsc{Tune Bottom-1} & 96.43 & -17.38 & 93.80 & -25.75 \\
%\testsc{Tune Bottom-3} & 96.43 & -17.38 & 93.80 & -25.75 \\

\testsc{Tune Bottom-3} & 96.43 & -17.38 & 95.82 & -18.50 \\
\testsc{Tune Bottom-5} & 96.43 & -17.38  & 96.34 & -17.70 \\
\testsc{Tune Bottom-8} & 96.43 & -17.38  & 96.62  & -17.29 \\
\testsc{Tune Bottom-10} & 96.43 & -17.38  & 96.31  & -17.05 \\
\hdashline
\multicolumn{1}{c}{\textit{Freezing encoder}}&\\
\testsc{Freeze Bottom-1} &  96.16 & -17.06 & 91.93 & -23.21 \\
\testsc{Freeze Bottom-3} &  96.34 & -16.70 & 94.39  & -18.49 \\
\testsc{Freeze Bottom-5} &  96.00 & -16.69 & 94.94 & -16.47 \\
%\testsc{Freeze Bottom-6} & & & 80.34 & 16.64 \\
\testsc{Freeze Bottom-8} & 94.87  & -17.39 & 93.94 & -16.29\\
\testsc{Freeze Bottom-10} & 92.68 & -17.70 & 92.58  & -17.09 \\
%\multicolumn{1}{c}{\textit{\reinit Decoder}}&\\
%\testsc{Encoder-7 + Decode-R}  & 94.60 & 80.34 & 16.64 \\
%\testsc{Encoder-9 + Decode-R}  & 94.94 & 79.98 & 15.29 \\

\midrule
&\multicolumn{3}{c}{\textit{NER}}\\


\standardFineTune & 83.09 &  -20.12 & - & - \\
\hdashline
\multicolumn{1}{c}{\textit{Fine-tuning all}}&\\
\testsc{Bottom-1} & 83.09 &  -20.12 & 69.88   & -25.31 \\
\testsc{Bottom-3} & 83.09 &  -20.12 &77.82  & -23.92 \\
\testsc{Bottom-6} & 83.09 &  -20.12 & 81.21 & -21.13 \\
\testsc{Bottom-8} & 83.09 &  -20.12 & 82.32 & -20.60 \\
\testsc{Bottom-10} & 83.09 & - 20.12 & 82.73 & -21.61\\

\hdashline
\multicolumn{1}{c}{\textit{Freezing encoder}}&\\
%\testsc{Fine-tune Encoder + Decode-R}  &82.25 &63.49& -21.67 \\

%\testsc{Freeze Bottom-3} & \\
\testsc{Freeze Bottom-1} & 82.40 & -19.12 & 66.07 & -26.03\\

\testsc{Freeze Bottom-3} & 83.19 & -18.50 & 73.19  & -21.38 \\
%\testsc{Freeze Bottom-5} & & &  & \\
\testsc{Freeze Bottom-6} &81.96 &18.01  & 76.89& -18.89\\
\testsc{Freeze Bottom-8} & 79.76 & -17.28 & 74.75 & -16.31\\
\testsc{Freeze Bottom-10} & 72.03  & -15.57  & 71.45 & -15.91 \\


%\hdashline
%\multicolumn{1}{c}{\textit{Pretrained Decoder}}&\\
%&&&&\\
%\multicolumn{1}{c}{\textit{\reinit Decoder}}&\\
%\testsc{Encoder-9 + Decode-R}  & 74.75 &  60.77 & 16.31 \\

\bottomrule


\end{tabular}
}
\caption{
%\textsc{Encoder-L} : L first layers of BERR frozen
%\textsc{Decoder} : 12-L layers self-attention layers pretrained of \reinit
}
\label{tab:re_init_x_freeze}
\end{table}


==> tables/freezing.tex <==







\begin{table}[t!]
\footnotesize\centering
\scalebox{0.80}{ % was .7775
\begin{tabular}{lrrrrrr}
    \toprule
    %Scenario  &
    &\multicolumn{3}{c}{\standardFineTune} & \multicolumn{3}{c}{Partial-Freezing}\\
     \cmidrule(l{2pt}c{0.3cm}){2-4}\cmidrule(l{2pt}c{0.3cm}){5-7}
    \textit{Task} &In-Lang& X-Lang & X-Sim & In-Lang& X-Lang & X-Sim \\
    \midrule
     %\\
    Parse & 89.05 & 52.90 & 72.92 & -0.04 &+0.85* & +0.56 \\%73.33
    %POS &  96.36 & 77.43 & 70.97 & +0.01 &+0.11 & +0.41\\ %71.35 \\%77.54 % 0.0006 &4.9*10-5
    POS &  96.36 & 77.43 & 70.97 & +0.01 &+0.22* & +0.41\\ %71.35 \\%77.54 % 0.0006 &4.9*10-5
    %POS &  96.60 & 77.78 & 70.97 & +0.02 &+0.25* & +0.38\\ %71.35 \\%77.54 % 0.0006 &4.9*10-5
    NER & 82.98 &59.86 &66.28 & -0.15&+2.12* & +4.75\\ %61.53&70.94\\%82.92-23.06  & 82.73-21.20 \\
    
\bottomrule


\end{tabular}
}
\caption{
Cross-Lingual Similarity (X-Sim) and \crosslang transfer (X-Lang) measured with \standardFineTune fine-tuned model and \partialfreezing (All the model is frozen except self-attention layer 3-11)
%\barre{Fine-tuning only 12 self-attention layers improve \similarity in the Fine-tuned models and improve \crosslang performance without hurting \inlang (In-Lang)\Djame{à mettre dans le texte}}
}
\label{tab:attention_freeze}
\end{table}

==> tables/pud_perf_freeze_vs_standart.tex <==





\begin{table*}[h!]
\footnotesize\centering
\scalebox{0.81}{ % was .7775
\begin{tabular}{lrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     
     &Evaluation&\textsc{\standardFineTune} & \textsc{Partial-Freezing} &
     %\textit{Re-Init.} & \textsc{None } & \textsc{0} & \textsc{1} & \textsc{2} & \textsc{5} & \textsc{8} & \textsc{10} & \textsc{11} & \textsc{0-1} & \textsc{1-2} & \textsc{2-3} & \textsc{4-5} & \textsc{6-7} & \textsc{8-9} & \textsc{10-11} & \textsc{0-2} & \textsc{1-3} & \textsc{4-6} & \textsc{9-11}  \\%& \\
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    \midrule
    
    

&& \multicolumn{2}{c}{\textit{Parsing}} \\

% PARSIn

\textit{\inlang} & \textsc{English} & 89.05 & 88.79 \\ 
\hdashline
 %\crosslang & \textsc{French} & 76.31 & 76.55 \\ 
 %& \textsc{German} & 72.72 & 73.34 \\ 
 %& \textsc{Russian} & 64.38 & 64.55 \\ 
 %& \textsc{Indonesian} & 48.17 & 49.21 \\ 
 %& \textsc{Arabic} & 36.62 & 40.01 \\ 
 %& \textsc{Porthughese} & 71.75 & 72.33 \\ 
 %& \textsc{SPanish} & 72.43 & 72.66 \\ 
 %& \textsc{Finish} & 50.79 & 50.38 \\ 
 %& \textsc{Italian} & 77.58 & 78.36 \\ 
 %& \textsc{Slovenian} & 75.32 & 74.96 \\ 
 %& \textsc{Czech} & 63.43 & 63.00 \\ 
 %& \textsc{Polish} & 58.43 & 58.42 \\ 
 %& \textsc{Hindi} & 30.96 & 31.81 \\ 
 %& \textsc{Chinese} & 31.99 & 32.36 \\ 
 %& \textsc{Turkish} & 33.02 & 32.80 \\ 
 %& \textsc{Japanese} & 15.29 & 16.59 \\ 
 %& \textsc{Thai} & 20.18 & 23.80 \\ 
 \textit{\crosslang} & \textsc{French} & 76.31 & 76.58 \\ 
 & \textsc{German} & 72.72 & 73.340\\ 
 & \textsc{Russian} & 64.38 & 64.50 \\ 
 & \textsc{Indonesian} & 48.17 & 49.20 \\ 
 & \textsc{Arabic} & 36.62 & 40.00 \\ 
 & \textsc{Porthughese} & 71.75 & 72.38 \\ 
 & \textsc{SPanish} & 72.43 & 72.61 \\ 
 & \textsc{Finish} & 50.79 & 50.15 \\ 
 & \textsc{Italian} & 77.58 & 78.31 \\ 
 & \textsc{Slovenian} & 75.32 & 75.00 \\ 
 & \textsc{Czech} & 63.43 & 63.01 \\ 
 & \textsc{Polish} & 58.43 & 58.43 \\ 
 & \textsc{Hindi} & 30.96 & 31.80 \\ 
 & \textsc{Chinese} & 31.99 & 32.35 \\ 
 & \textsc{Turkish} & 33.02 & 32.70 \\ 
 & \textsc{Japanese} & 15.29 & 16.68 \\ 
 & \textsc{Thai} & 20.18 & 23.81 \\ 
%& Avg  & 54.91 & -0.64 \\ 
\hdashline
\textit{Summary} & \gap & -36.15 & -35.09 \\ 
\midrule
&& \multicolumn{2}{c}{\textit{POS}} \\

% POS
 \textit{\inlang} & \textsc{English} & 96.31 & 96.32 \\ 
 \hdashline
 %\crosslang & \textsc{French} & 89.27 & 89.33 \\ 
 %& \textsc{German} & 89.25 & 89.26 \\ 
 %& \textsc{Russian} & 87.26 & 86.47 \\ 
 %& \textsc{Indonesian} & 71.93 & 73.31 \\ 
 %& \textsc{Arabic} & 67.68 & 67.01 \\ 
 %& \textsc{Porthughese} & 86.88 & 86.95 \\ 
 %& \textsc{SPanish} & 87.61 & 87.63 \\ 
 %& \textsc{Finish} & 84.69 & 85.23 \\ 
 %& \textsc{Italian} & 91.33 & 91.59 \\ 
 %& \textsc{Slovenian} & 90.56 & 90.99 \\ 
 %& \textsc{Czech} & 83.47 & 82.30 \\ 
 %& \textsc{Polish} & 82.08 & 82.48 \\ 
 %& \textsc{Hindi} & 67.49 & 66.53 \\ 
 %& \textsc{Chinese} & 67.87 & 66.33 \\ 
 %& \textsc{Turkish} & 68.54 & 69.32 \\ 
 %& \textsc{Japanese} & 48.77 & 49.30 \\ 
 %& \textsc{Thai} & 51.57 & 54.20 \\ 
%& Avg  & 78.48 & -0.11 \\ 
\textit{\crosslang} & \textsc{French} & 89.27 & 89.43 \\ 
 & \textsc{German} & 89.25 & 89.23 \\ 
 & \textsc{Russian} & 87.26 & 86.70 \\ 
 & \textsc{Indonesian} & 71.93 & 73.61 \\ 
 & \textsc{Arabic} & 67.68 & 67.11 \\ 
 & \textsc{Porthughese} & 86.88 & 86.91 \\ 
 & \textsc{SPanish} & 87.61 & 87.67 \\ 
 & \textsc{Finish} & 84.69 & 85.41 \\ 
 & \textsc{Italian} & 91.33 & 91.61 \\ 
 & \textsc{Slovenian} & 90.56 & 90.99 \\ 
 & \textsc{Czech} & 83.47 & 82.49 \\ 
 & \textsc{Polish} & 82.08 & 82.69 \\ 
 & \textsc{Hindi} & 67.49 & 66.73 \\ 
 & \textsc{Chinese} & 67.87 & 66.63 \\ 
 & \textsc{Turkish} & 68.54 & 69.52 \\ 
 & \textsc{Japanese} & 48.77 & 49.41 \\ 
 & \textsc{Thai} & 51.57 & 54.19 \\ 
\hdashline
\textit{Summary} & \gap & -18.88 & -18.67 \\ 
\midrule
&& \multicolumn{2}{c}{\textit{NER}} \\

% NER
 \textit{\inlang}& \textsc{English} & 82.98 & 82.83 \\ 
 \hdashline
 %\crosslang& \textsc{French} & 76.81 & 78.40 \\ 
 %& \textsc{German} & 76.39 & 77.84 \\ 
 %& \textsc{Russian} & 58.59 & 62.21 \\ 
 %& \textsc{Indonesian} & 54.44 & 57.99 \\ 
 %& \textsc{Arabic} & 43.88 & 39.94 \\ 
 %& \textsc{Porthughese} & 77.02 & 78.36 \\ 
 %& \textsc{SPanish} & 68.49 & 70.92 \\ 
 %& \textsc{Finish} & 76.13 & 77.73 \\ 
 %& \textsc{Italian} & 78.72 & 79.90 \\ 
 %& \textsc{Slovenian} & 68.86 & 72.99 \\ 
 %& \textsc{Czech} & 78.09 & 79.78 \\ 
 %& \textsc{Polish} & 77.80 & 77.99 \\ 
 %& \textsc{Chinese} & 38.53 & 41.98 \\ 
 %& \textsc{Japanese} & 24.87 & 25.65 \\ 
 %& \textsc{Hindi} & 60.92 & 65.30 \\ 
 %& \textsc{Thai} & 0.35 & 0.66 \\ 
 %& \textsc{Turkish} & 57.64 & 59.71 \\ 
 \textit{\crosslang}& \textsc{French} & 76.81 & 78.40 \\ 
 & \textsc{German} & 76.39 & 77.84 \\ 
 & \textsc{Russian} & 58.59 & 62.21 \\ 
 & \textsc{Indonesian} & 54.44 & 57.99 \\ 
 & \textsc{Arabic} & 43.88 & 39.94 \\ 
 & \textsc{Porthughese} & 77.02 & 78.36 \\ 
 & \textsc{SPanish} & 68.49 & 70.92 \\ 
 & \textsc{Finish} & 76.13 & 77.73 \\ 
 & \textsc{Italian} & 78.72 & 79.90 \\ 
 & \textsc{Slovenian} & 68.86 & 72.99 \\ 
 & \textsc{Czech} & 78.09 & 79.78 \\ 
 & \textsc{Polish} & 77.80 & 77.99 \\ 
 & \textsc{Chinese} & 38.53 & 41.98 \\ 
 & \textsc{Japanese} & 24.87 & 25.65 \\ 
 & \textsc{Hindi} & 60.92 & 65.30 \\ 
 & \textsc{Thai} & 0.35 & 0.66 \\ 
 & \textsc{Turkish} & 57.64 & 59.71 \\ 
%& Avg  & 61.14 & -1.57 \\
\hdashline
\textit{Summary} & \gap & -23.12 & -21.20 \\ 
\bottomrule

\end{tabular}
}
\caption{Zero shot cross-lingual performances when partially-freezing the model compared to the \standardFineTune fine-tuned model. Partial-freeze corresponds to a model for which we only fine-tuned the self-attention of layers 3-11 and the randomly-initialized head. For all target languages, reporting scores on test split.
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Each score is the average of 5 runs with different random seeds.\\
Std  min/median/max Parsing:0.03/0.23/1.52, POS:0.01/0.11/1.02, NER:0.0/0.45/1.62%\ye{is he appendix?}
}
\label{tab:partial_freezing_details}%re_init_x4_all_reduce}
\end{table*}

==> tables/pud_performances.tex <==


% PARSING 

\textsc{English} & 89.05 \\ 
\textsc{French} & \cellcolor{green}76.31 \\ 
\textsc{German} & \cellcolor{green}72.72 \\ 
\textsc{Russian} & \cellcolor{green}64.38 \\ 
\textsc{Indo} & \cellcolor{green}48.17 \\ 
\textsc{Arabic} & \cellcolor{green}36.62 \\ 
\textsc{Porthughese} & \cellcolor{green}71.75 \\ 
\textsc{SPanish} & \cellcolor{green}72.43 \\ 
\textsc{Finish} & \cellcolor{green}50.79 \\ 
\textsc{Italian} & \cellcolor{green}77.58 \\ 
\textsc{Slovenian} & \cellcolor{green}75.32 \\ 
\textsc{Czech} & \cellcolor{green}63.43 \\ 
\textsc{Polish} & \cellcolor{green}58.43 \\ 
\textsc{Hindi} & \cellcolor{green}30.96 \\ 
\textsc{Chinese} & \cellcolor{green}31.99 \\ 
\textsc{Turkish} & \cellcolor{green}33.02 \\ 
\textsc{Japanese} & \cellcolor{green}15.29 \\ 
\textsc{Thai} & \cellcolor{green}20.18 \\ 
& Avg  & 54.91 \\ 
Summary & \textsc{CL Transfer Gap}  & 36.15 \\ 

%POS 
\textsc{English} & 96.54 \\ 
\textsc{French} & \cellcolor{green}89.77 \\ 
\textsc{German} & \cellcolor{green}89.25 \\ 
\textsc{Russian} & \cellcolor{green}87.26 \\ 
\textsc{Indo} & \cellcolor{green}71.93 \\ 
\textsc{Arabic} & \cellcolor{green}67.68 \\ 
\textsc{Porthughese} & \cellcolor{green}86.88 \\ 
\textsc{SPanish} & \cellcolor{green}87.61 \\ 
\textsc{Finish} & \cellcolor{green}85.89 \\ 
\textsc{Italian} & \cellcolor{green}91.83 \\ 
\textsc{Slovenian} & \cellcolor{green}90.56 \\ 
\textsc{Czech} & \cellcolor{green}84.27 \\ 
\textsc{Polish} & \cellcolor{green}82.08 \\ 
\textsc{Hindi} & \cellcolor{green}67.49 \\ 
\textsc{Chinese} & \cellcolor{green}67.87 \\ 
\textsc{Turkish} & \cellcolor{green}68.54 \\ 
\textsc{Japanese} & \cellcolor{green}51.27 \\ 
\textsc{Thai} & \cellcolor{green}45.07 \\ 
& Avg  & 78.43 \\ 
Summary & \textsc{CL Transfer Gap}  & 19.17 \\


% NER 

\textsc{English} & 82.92 \\ 
\textsc{French} & \cellcolor{green}76.81 \\ 
\textsc{German} & \cellcolor{green}76.39 \\ 
\textsc{Russian} & \cellcolor{green}58.59 \\ 
\textsc{Indo} & \cellcolor{green}54.44 \\ 
\textsc{Arabic} & \cellcolor{green}43.88 \\ 
\textsc{Porthughese} & \cellcolor{green}77.02 \\ 
\textsc{SPanish} & \cellcolor{green}68.49 \\ 
\textsc{Finish} & \cellcolor{green}76.13 \\ 
\textsc{Italian} & \cellcolor{green}78.72 \\ 
\textsc{Slovenian} & \cellcolor{green}68.86 \\ 
\textsc{Czech} & \cellcolor{green}78.09 \\ 
\textsc{Polish} & \cellcolor{green}77.80 \\ 
\textsc{Hindi} & \cellcolor{green}60.92 \\ 
\textsc{Chinese} & \cellcolor{green}38.53 \\ 
\textsc{Turkish} & \cellcolor{green}57.64 \\ 
\textsc{Japanese} & \cellcolor{green}24.87 \\ 
\textsc{Thai} & \cellcolor{green}0.35 \\ 
& Avg  & 61.14 \\ 
Summary & \textsc{CL Transfer Gap}  & 23.06 \\ 

==> tables/re_init_abs_table.tex <==




\begin{table*}[h!]
\footnotesize\centering
\scalebox{0.85}{ % was .7775
\begin{tabular}{llrrrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     &&  \multicolumn{9}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     Setting&Eval&\textsc{\standardFineTune} & \textsc{All} & \textsc{0} & \textsc{1} & \textsc{0-1} & \textsc{2-3} &  \textsc{0-3} & \textsc{4-7} & \textsc{8-11} &
     %\textit{Re-Init.} & \textsc{None } & \textsc{0} & \textsc{1} & \textsc{2} & \textsc{5} & \textsc{8} & \textsc{10} & \textsc{11} & \textsc{0-1} & \textsc{1-2} & \textsc{2-3} & \textsc{4-5} & \textsc{6-7} & \textsc{8-9} & \textsc{10-11} & \textsc{0-2} & \textsc{1-3} & \textsc{4-6} & \textsc{9-11}  \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    \midrule

&&  \multicolumn{9}{c}{\textit{Parsing}} \\
  & \textsc{English} & 88.62 & \cellcolor{brightlavender}74.58 & \cellcolor{lightgreen}87.77 & \cellcolor{lightgreen}88.09 & \cellcolor{lightgreen}87.25 & \cellcolor{lightgreen}86.79 & \cellcolor{pink}83.10 & \cellcolor{lightgreen}85.37 & \cellcolor{mediumspringgreen}88.69 \\ 
 & \textsc{French} & 68.86 & \cellcolor{brightlavender}3.70 & \cellcolor{lightgreen}65.73 & \cellcolor{lightgreen}65.21 & \cellcolor{brightlavender}55.31 & \cellcolor{pink}61.31 & \cellcolor{brightlavender}37.29 & \cellcolor{pink}61.82 & \cellcolor{mediumspringgreen}69.26 \\ 
 & \textsc{German} & 67.53 & \cellcolor{brightlavender}4.73 & \cellcolor{lightgreen}64.97 & \cellcolor{lightgreen}65.20 & \cellcolor{brightlavender}57.08 & \cellcolor{pink}60.62 & \cellcolor{brightlavender}36.05 & \cellcolor{pink}59.37 & \cellcolor{lightgreen}67.21 \\ 
 & \textsc{Turkish} & 28.37 & \cellcolor{brightlavender}2.76 & \cellcolor{pink}21.65 & \cellcolor{lightgreen}23.77 & \cellcolor{brightlavender}16.78 & \cellcolor{pink}21.21 & \cellcolor{brightlavender}9.70 & \cellcolor{pink}20.94 & \cellcolor{mediumspringgreen}29.33 \\ 
 & \textsc{Indonesian} & 45.19 & \cellcolor{brightlavender}4.99 & \cellcolor{lightgreen}43.33 & \cellcolor{lightgreen}43.48 & \cellcolor{pink}39.83 & \cellcolor{pink}39.09 & \cellcolor{brightlavender}30.35 & \cellcolor{lightgreen}40.85 & \cellcolor{mediumspringgreen}47.53 \\ 
 & \textsc{Russian} & 59.57 & \cellcolor{brightlavender}2.95 & \cellcolor{lightgreen}57.81 & \cellcolor{lightgreen}57.53 & \cellcolor{pink}54.10 & \cellcolor{pink}53.51 & \cellcolor{brightlavender}38.58 & \cellcolor{pink}52.41 & \cellcolor{mediumspringgreen}60.72 \\ 
 & \textsc{Arabic} & 23.51 & \cellcolor{brightlavender}3.19 & \cellcolor{mediumspringgreen}23.66 & \cellcolor{lightgreen}23.49 & \cellcolor{lightgreen}21.01 & \cellcolor{lightgreen}19.55 & \cellcolor{brightlavender}13.26 & \cellcolor{pink}18.27 & \cellcolor{mediumspringgreen}23.93 \\ 
Summary & \textsc{CL Transfer Gap}  & -39.78 & -70.86 & -41.57 & -41.65 & -46.56 & -44.24 & -55.56 & -43.10 & -39.02 \\




\midrule
&&  \multicolumn{9}{c}{\textit{POS}} \\
  & \textsc{English} & 96.47 & \cellcolor{pink}87.71 & \cellcolor{lightgreen}96.08 & \cellcolor{lightgreen}96.24 & \cellcolor{lightgreen}95.94 & \cellcolor{lightgreen}95.72 & \cellcolor{lightgreen}94.05 & \cellcolor{lightgreen}95.45 & \cellcolor{mediumspringgreen}96.51 \\ 
 & \textsc{French} & 88.23 & \cellcolor{brightlavender}28.96 & \cellcolor{lightgreen}86.70 & \cellcolor{lightgreen}87.66 & \cellcolor{pink}79.84 & \cellcolor{lightgreen}87.14 & \cellcolor{brightlavender}62.28 & \cellcolor{lightgreen}86.37 & \cellcolor{mediumspringgreen}88.26 \\ 
 & \textsc{German} & 90.51 & \cellcolor{brightlavender}28.93 & \cellcolor{lightgreen}88.26 & \cellcolor{lightgreen}89.53 & \cellcolor{pink}82.26 & \cellcolor{lightgreen}88.39 & \cellcolor{brightlavender}59.16 & \cellcolor{lightgreen}89.12 & \cellcolor{mediumspringgreen}90.64 \\ 
 & \textsc{Turkish} & 72.49 & \cellcolor{brightlavender}32.23 & \cellcolor{brightlavender}62.17 & \cellcolor{pink}66.17 & \cellcolor{brightlavender}54.50 & \cellcolor{pink}63.22 & \cellcolor{brightlavender}44.16 & \cellcolor{lightgreen}69.30 & \cellcolor{mediumspringgreen}73.08 \\ 
 & \textsc{Indonesian} & 84.02 & \cellcolor{brightlavender}36.98 & \cellcolor{lightgreen}82.15 & \cellcolor{lightgreen}82.89 & \cellcolor{lightgreen}80.13 & \cellcolor{lightgreen}81.40 & \cellcolor{brightlavender}72.42 & \cellcolor{lightgreen}82.59 & \cellcolor{mediumspringgreen}84.09 \\ 
 & \textsc{Russian} & 83.04 & \cellcolor{brightlavender}32.63 & \cellcolor{mediumspringgreen}83.14 & \cellcolor{mediumspringgreen}83.63 & \cellcolor{lightgreen}81.95 & \cellcolor{lightgreen}82.26 & \cellcolor{brightlavender}70.33 & \cellcolor{lightgreen}82.56 & \cellcolor{mediumspringgreen}83.19 \\ 
 & \textsc{Arabic} & 56.44 & \cellcolor{brightlavender}19.61 & \cellcolor{mediumspringgreen}58.10 & \cellcolor{mediumspringgreen}58.06 & \cellcolor{mediumspringgreen}57.89 & \cellcolor{lightgreen}55.62 & \cellcolor{lightgreen}52.28 & \cellcolor{lightgreen}53.60 & \cellcolor{mediumspringgreen}58.84 \\ 
Summary & \textsc{CL Transfer Gap}  & -17.35 & -57.82 & -19.32 & -18.25 & -23.18 & -19.38 & -33.95 & -18.19 & -16.83 \\ 
\midrule

&&  \multicolumn{9}{c}{\textit{NER}} \\

 & \textsc{English} & 82.98 & \cellcolor{brightlavender}56.56 & \cellcolor{lightgreen}81.46 & \cellcolor{lightgreen}82.00 & \cellcolor{lightgreen}79.63 & \cellcolor{lightgreen}79.25 & \cellcolor{brightlavender}69.08 & \cellcolor{lightgreen}79.91 & \cellcolor{lightgreen}82.27 \\ 
 & \textsc{French} & 76.65 & \cellcolor{brightlavender}35.35 & \cellcolor{lightgreen}75.46 & \cellcolor{mediumspringgreen}77.57 & \cellcolor{pink}69.94 & \cellcolor{lightgreen}72.83 & \cellcolor{brightlavender}55.79 & \cellcolor{lightgreen}73.12 & \cellcolor{lightgreen}75.77 \\ 
 & \textsc{German} & 76.35 & \cellcolor{brightlavender}18.95 & \cellcolor{lightgreen}73.73 & \cellcolor{lightgreen}75.39 & \cellcolor{brightlavender}66.18 & \cellcolor{pink}70.12 & \cellcolor{brightlavender}42.37 & \cellcolor{pink}71.14 & \cellcolor{lightgreen}75.50 \\ 
 & \textsc{Turkish} & 67.45 & \cellcolor{brightlavender}20.76 & \cellcolor{lightgreen}62.54 & \cellcolor{lightgreen}64.84 & \cellcolor{brightlavender}52.20 & \cellcolor{brightlavender}57.11 & \cellcolor{brightlavender}39.38 & \cellcolor{pink}61.43 & \cellcolor{lightgreen}66.62 \\ 
 & \textsc{Indo} & 54.10 & \cellcolor{brightlavender}21.20 & \cellcolor{lightgreen}49.19 & \cellcolor{lightgreen}49.27 & \cellcolor{pink}46.50 & \cellcolor{pink}46.87 & \cellcolor{brightlavender}36.11 & \cellcolor{pink}46.06 & \cellcolor{pink}48.23 \\ 
 & \textsc{Russian} & 58.28 & \cellcolor{brightlavender}7.43 & \cellcolor{lightgreen}55.63 & \cellcolor{lightgreen}58.08 & \cellcolor{pink}50.67 & \cellcolor{pink}52.89 & \cellcolor{brightlavender}34.66 & \cellcolor{pink}52.03 & \cellcolor{mediumspringgreen}59.12 \\ 
 & \textsc{Arabic} & 41.88 & \cellcolor{brightlavender}5.49 & \cellcolor{pink}35.79 & \cellcolor{pink}34.80 & \cellcolor{pink}32.37 & \cellcolor{pink}32.31 & \cellcolor{brightlavender}21.85 & \cellcolor{lightgreen}38.67 & \cellcolor{lightgreen}41.23 \\ 
Summary & \textsc{CL Transfer Gap}  & -20.53 & -38.37 & -22.74 & -22.01 & -26.65 & -23.89 & -30.72 & -22.83 & -21.20 \\ 

\bottomrule

\end{tabular}
}
\caption{Absolute Zero shot Cross-Lingual performance compared to reference (\textsc{Ref} column) when fine-tuning the model applying  \reinit (section \ref{sec:controlled_exp}) to specific set of layers. Source language is English. Baseline \textsc{ALL} (for all layers randomly initialized) corresponds to a model trained from scratch on the task.
\textsc{Ref} column is model \standardFineTune fine-tuned model. 
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Std min/median/max, Parsing:0.02/0.34/1.48,POS:0.01/0.5/2.38,NER:0.0/0.47/2.62
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
}
\label{tab:re_init_x4_all_reduce_appendix}%re_init_x4_all_reduce}
\end{table*}

==> tables/re_init_table.tex <==


\begin{table*}[h!]
\footnotesize\centering
\scalebox{0.78}{ % was .7775
\begin{tabular}{llrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     && & \multicolumn{4}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     Setting&Eval&\textsc{\standardFineTune} & \textsc{All} & \textsc{0-3} & \textsc{4-7} & \textsc{8-11} &
     %\textit{Re-Init.} & \textsc{None } & \textsc{0} & \textsc{1} & \textsc{2} & \textsc{5} & \textsc{8} & \textsc{10} & \textsc{11} & \textsc{0-1} & \textsc{1-2} & \textsc{2-3} & \textsc{4-5} & \textsc{6-7} & \textsc{8-9} & \textsc{10-11} & \textsc{0-2} & \textsc{1-3} & \textsc{4-6} & \textsc{9-11}  \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    \midrule
&&\multicolumn{5}{c}{\textit{Parsing}}\\
 
\inlang& \textsc{English} & 88.62 & \cellcolor{red}-14.04 & \cellcolor{pink}-5.52 & \cellcolor{lightgreen}-3.25 & \cellcolor{green}0.07 \\ 
\hdashline
 \crosslang& \textsc{French} & \cellcolor{green}68.92 & \cellcolor{red}-65.22 & \cellcolor{red}-31.63 & \cellcolor{pink}-7.10 & \cellcolor{green}0.34 \\ 
 & \textsc{German} & \cellcolor{green}67.92 & \cellcolor{red}-63.19 & \cellcolor{red}-31.86 & \cellcolor{pink}-8.54 & \cellcolor{lightgreen}-0.71 \\ 
 & \textsc{Turkish} & \cellcolor{green}28.46 & \cellcolor{red}-25.70 & \cellcolor{red}-18.76 & \cellcolor{pink}-7.52 & \cellcolor{green}0.88 \\ 
 & \textsc{Indonesian} & \cellcolor{green}45.26 & \cellcolor{red}-40.27 & \cellcolor{red}-14.90 & \cellcolor{lightgreen}-4.40 & \cellcolor{green}2.28 \\ 
 & \textsc{Russian} & \cellcolor{green}59.30 & \cellcolor{red}-56.35 & \cellcolor{red}-20.71 & \cellcolor{pink}-6.89 & \cellcolor{green}1.43 \\ 
 & \textsc{Arabic} & \cellcolor{green}23.41 & \cellcolor{red}-20.22 & \cellcolor{red}-10.16 & \cellcolor{pink}-5.15 & \cellcolor{green}0.52 \\ 
%&Avg  & 54.55 & -40.71 & -19.08 & -6.12 & 0.69 \\ 
\hdashline
Summary & Avg \gap  & \cellcolor{green}-39.74 &\cellcolor{darkred} -70.86 & \cellcolor{red}-55.56 & \cellcolor{lightgreen}-43.10 & \cellcolor{green}-39.02 \\

\midrule
&&\multicolumn{5}{c}{\textit{POS}}\\

 \inlang& \textsc{English} & 96.43 & \cellcolor{pink}-8.73 & \cellcolor{lightgreen}-2.38 & \cellcolor{lightgreen}-0.98 & \cellcolor{green}0.08 \\ 
 \hdashline
 \crosslang& \textsc{French} & \cellcolor{green}88.33 & \cellcolor{red}-59.37 & \cellcolor{red}-26.05 & \cellcolor{lightgreen}-1.96 & \cellcolor{lightgreen}-0.06 \\ 
 & \textsc{German} & \cellcolor{green}90.22 & \cellcolor{red}-61.29 & \cellcolor{red}-31.06 & \cellcolor{lightgreen}-1.10 & \cellcolor{green}0.42 \\ 
 & \textsc{Turkish} & \cellcolor{green}72.31 & \cellcolor{red}-40.08 & \cellcolor{red}-28.15 & \cellcolor{lightgreen}-3.01 & \cellcolor{green}0.77 \\ 
 & \textsc{Indonesian} & \cellcolor{green}83.91 & \cellcolor{red}-46.93 & \cellcolor{red}-11.49 & \cellcolor{lightgreen}-1.32 & \cellcolor{green}0.18 \\ 
 & \textsc{Russian} & \cellcolor{green}83.11 & \cellcolor{red}-50.49 & \cellcolor{red}-12.79 & \cellcolor{lightgreen}-0.55 & \cellcolor{green}0.07 \\ 
 & \textsc{Arabic} & \cellcolor{green}56.45 & \cellcolor{red}-36.84 & \cellcolor{lightgreen}-4.18 & \cellcolor{lightgreen}-2.85 & \cellcolor{green}2.38 \\ 
%&Avg  & 81.54 & -43.39 & -16.59 & -1.68 & 0.55 \\ 
\hdashline
Summary & Avg \gap  & \cellcolor{green}-17.38 & \cellcolor{darkred}-57.82 & \cellcolor{red}-33.95 & \cellcolor{lightgreen}-18.19 & \cellcolor{green} -16.83 \\ 


\midrule
&&\multicolumn{5}{c}{\textit{NER}}\\
 \inlang & \textsc{English} & 83.09 & \cellcolor{red}-26.52 & \cellcolor{red}-14.00 & \cellcolor{lightgreen}-3.18 & \cellcolor{lightgreen}-0.81 \\ 
 \hdashline
 \crosslang& \textsc{French} & \cellcolor{green}76.81 & \cellcolor{red}-41.46 & \cellcolor{red}-21.02 & \cellcolor{lightgreen}-3.68 & \cellcolor{lightgreen}-1.04 \\ 
 & \textsc{German} & \cellcolor{green}76.39 & \cellcolor{red}-57.44 & \cellcolor{red}-34.02 & \cellcolor{pink}-5.25 & \cellcolor{lightgreen}-0.90 \\ 
 & \textsc{Turkish} & \cellcolor{green}67.66 & \cellcolor{red}-46.90 & \cellcolor{red}-28.28 & \cellcolor{pink}-6.22 & \cellcolor{lightgreen}-1.04 \\ 
 
 & \textsc{Indonesian} & \cellcolor{green}54.44 & \cellcolor{red}-33.23 & \cellcolor{red}-18.33 & \cellcolor{pink}-8.38 & \cellcolor{pink}-6.20 \\ 
 & \textsc{Russian} & \cellcolor{green}58.59 & \cellcolor{red}-51.16 & \cellcolor{red}-23.94 & \cellcolor{pink}-6.56 & \cellcolor{green}0.53 \\ 
 & \textsc{Arabic} & \cellcolor{green}43.88 & \cellcolor{red}-38.39 & \cellcolor{red}-22.03 & \cellcolor{pink}-5.20 & \cellcolor{lightgreen}-2.65 \\ 
& Avg  & 65.84 & -42.16 & -23.09 & -5.50 & -1.73 \\ 
\hdashline
Summary & Avg \gap  & -20.12 & \cellcolor{darkred}-38.37 &\cellcolor{red} -30.72 & \cellcolor{lightgreen}-22.83 & \cellcolor{lightgreen}-21.20 \\ 

\bottomrule

\end{tabular}
}
\caption{Relative Zero shot Cross-Lingual performance compared to reference (\textsc{Ref} column) when fine-tuning the model applying  \reinit (section \ref{sec:controlled_exp}) to specific set of layers. Source language is English. Baseline \textsc{ALL} (for all layers randomly initialized) corresponds to a model trained from scratch on the task.
\textsc{Ref} column is model \standardFineTune fine-tuned model. 
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Std min/median/max NER:0.0/0.47/2.62
\bm{add std for all}
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
}
\label{tab:re_init_x4_all_reduce}%re_init_x4_all_reduce}
\end{table*}

==> tables/re_init_table_with_x1_x2.tex <==




\begin{table*}[h!]
\footnotesize\centering
\scalebox{0.85}{ % was .7775
\begin{tabular}{llrrrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     &&  \multicolumn{9}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     Setting&Eval&\textsc{\standardFineTune} & \textsc{All} & \textsc{0} & \textsc{1} & \textsc{0-1} &
     \textsc{2-3} &  \textsc{0-3} & \textsc{4-7} & \textsc{8-11} &
     %\textit{Re-Init.} & \textsc{None } & \textsc{0} & \textsc{1} & \textsc{2} & \textsc{5} & \textsc{8} & \textsc{10} & \textsc{11} & \textsc{0-1} & \textsc{1-2} & \textsc{2-3} & \textsc{4-5} & \textsc{6-7} & \textsc{8-9} & \textsc{10-11} & \textsc{0-2} & \textsc{1-3} & \textsc{4-6} & \textsc{9-11}  \\%& \\
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    \midrule

&&  \multicolumn{9}{c}{\textit{Parsing}} \\
  \inlang & \textsc{English} & 88.62 & \cellcolor{brightlavender}-14.04 & \cellcolor{lightgreen}-0.85 & \cellcolor{lightgreen}-0.52 & \cellcolor{lightgreen}-1.37 & \cellcolor{lightgreen}-1.83 & \cellcolor{pink}-5.51 & \cellcolor{lightgreen}-3.24 & \cellcolor{mediumspringgreen}0.07 \\ 
\hdashline
 \crosslang& \textsc{French} & 68.86 & \cellcolor{brightlavender}-65.16 & \cellcolor{lightgreen}-3.14 & \cellcolor{lightgreen}-3.65 & \cellcolor{brightlavender}-13.55 & \cellcolor{pink}-7.55 & \cellcolor{brightlavender}-31.58 & \cellcolor{pink}-7.04 & \cellcolor{mediumspringgreen}0.40 \\ 
 & \textsc{German} & 67.53 & \cellcolor{brightlavender}-62.80 & \cellcolor{lightgreen}-2.55 & \cellcolor{lightgreen}-2.33 & \cellcolor{brightlavender}-10.44 & \cellcolor{pink}-6.91 & \cellcolor{brightlavender}-31.47 & \cellcolor{pink}-8.15 & \cellcolor{lightgreen}-0.32 \\ 
 & \textsc{Turkish} & 28.37 & \cellcolor{brightlavender}-25.61 & \cellcolor{pink}-6.71 & \cellcolor{lightgreen}-4.60 & \cellcolor{brightlavender}-11.58 & \cellcolor{pink}-7.16 & \cellcolor{brightlavender}-18.67 & \cellcolor{pink}-7.43 & \cellcolor{mediumspringgreen}0.97 \\ 
 & \textsc{Indonesian} & 45.19 & \cellcolor{brightlavender}-40.20 & \cellcolor{lightgreen}-1.86 & \cellcolor{lightgreen}-1.71 & \cellcolor{pink}-5.36 & \cellcolor{pink}-6.10 & \cellcolor{brightlavender}-14.84 & \cellcolor{lightgreen}-4.34 & \cellcolor{mediumspringgreen}2.34 \\ 
 & \textsc{Russian} & 59.57 & \cellcolor{brightlavender}-56.63 & \cellcolor{lightgreen}-1.76 & \cellcolor{lightgreen}-2.04 & \cellcolor{pink}-5.47 & \cellcolor{pink}-6.06 & \cellcolor{brightlavender}-20.99 & \cellcolor{pink}-7.17 & \cellcolor{mediumspringgreen}1.15 \\ 
 & \textsc{Arabic} & 23.51 & \cellcolor{brightlavender}-20.32 & \cellcolor{mediumspringgreen}0.15 & \cellcolor{lightgreen}-0.02 & \cellcolor{lightgreen}-2.50 & \cellcolor{lightgreen}-3.95 & \cellcolor{brightlavender}-10.25 & \cellcolor{pink}-5.24 & \cellcolor{mediumspringgreen}0.42 \\ 
 \hdashline
Summary & \gap  & -39.78 & \cellcolor{brightlavender}-70.86 & \cellcolor{lightgreen}-41.57 & \cellcolor{lightgreen}-41.65 & \cellcolor{pink}-46.56 & \cellcolor{pink}-44.24 & \cellcolor{brightlavender}-55.56 & \cellcolor{pink}-43.10 & \cellcolor{green}-39.02 \\ 
\midrule

&&  \multicolumn{9}{c}{\textit{POS}} \\

 & \textsc{English} & 96.47 & \cellcolor{pink}-8.76 & \cellcolor{lightgreen}-0.39 & \cellcolor{lightgreen}-0.23 & \cellcolor{lightgreen}-0.53 & \cellcolor{lightgreen}-0.75 & \cellcolor{lightgreen}-2.42 & \cellcolor{lightgreen}-1.02 & \cellcolor{mediumspringgreen}0.04 \\ 
 & \textsc{French} & 88.23 & \cellcolor{brightlavender}-59.28 & \cellcolor{lightgreen}-1.53 & \cellcolor{lightgreen}-0.57 & \cellcolor{pink}-8.39 & \cellcolor{lightgreen}-1.09 & \cellcolor{brightlavender}-25.96 & \cellcolor{lightgreen}-1.86 & \cellcolor{mediumspringgreen}0.03 \\ 
 & \textsc{German} & 90.51 & \cellcolor{brightlavender}-61.59 & \cellcolor{lightgreen}-2.25 & \cellcolor{lightgreen}-0.98 & \cellcolor{pink}-8.25 & \cellcolor{lightgreen}-2.13 & \cellcolor{brightlavender}-31.35 & \cellcolor{lightgreen}-1.39 & \cellcolor{mediumspringgreen}0.13 \\ 
 & \textsc{Turkish} & 72.49 & \cellcolor{brightlavender}-40.26 & \cellcolor{brightlavender}-10.32 & \cellcolor{pink}-6.32 & \cellcolor{brightlavender}-17.99 & \cellcolor{pink}-9.27 & \cellcolor{brightlavender}-28.33 & \cellcolor{lightgreen}-3.19 & \cellcolor{mediumspringgreen}0.59 \\ 
 & \textsc{Indonesian} & 84.02 & \cellcolor{brightlavender}-47.04 & \cellcolor{lightgreen}-1.86 & \cellcolor{lightgreen}-1.12 & \cellcolor{lightgreen}-3.88 & \cellcolor{lightgreen}-2.61 & \cellcolor{brightlavender}-11.60 & \cellcolor{lightgreen}-1.43 & \cellcolor{mediumspringgreen}0.07 \\ 
 & \textsc{Russian} & 83.04 & \cellcolor{brightlavender}-50.41 & \cellcolor{mediumspringgreen}0.10 & \cellcolor{mediumspringgreen}0.59 & \cellcolor{lightgreen}-1.09 & \cellcolor{lightgreen}-0.78 & \cellcolor{brightlavender}-12.71 & \cellcolor{lightgreen}-0.48 & \cellcolor{mediumspringgreen}0.15 \\ 
 & \textsc{Arabic} & 56.44 & \cellcolor{brightlavender}-36.83 & \cellcolor{mediumspringgreen}1.66 & \cellcolor{mediumspringgreen}1.62 & \cellcolor{mediumspringgreen}1.45 & \cellcolor{lightgreen}-0.82 & \cellcolor{lightgreen}-4.17 & \cellcolor{lightgreen}-2.84 & \cellcolor{mediumspringgreen}2.39 \\ 
Summary & \textsc{CL Transfer Gap}  & -17.35 & -57.82 & -19.32 & -18.25 & -23.18 & -19.38 & -33.95 & -18.19 & -16.83 \\ 
\midrule

&&  \multicolumn{9}{c}{\textit{NER}} \\
 \inlang & \textsc{English} & 82.98 & \cellcolor{brightlavender}-26.42 & \cellcolor{lightgreen}-1.52 & \cellcolor{lightgreen}-0.98 & \cellcolor{lightgreen}-3.35 & \cellcolor{lightgreen}-3.73 & \cellcolor{brightlavender}-13.90 & \cellcolor{lightgreen}-3.08 & \cellcolor{lightgreen}-0.71 \\ 
\hdashline
 \crosslang& \textsc{French} & 76.65 & \cellcolor{brightlavender}-41.30 & \cellcolor{lightgreen}-1.19 & \cellcolor{mediumspringgreen}0.92 & \cellcolor{pink}-6.71 & \cellcolor{lightgreen}-3.82 & \cellcolor{brightlavender}-20.86 & \cellcolor{lightgreen}-3.53 & \cellcolor{lightgreen}-0.88 \\ 
 & \textsc{German} & 76.35 & \cellcolor{brightlavender}-57.39 & \cellcolor{lightgreen}-2.62 & \cellcolor{lightgreen}-0.96 & \cellcolor{brightlavender}-10.17 & \cellcolor{pink}-6.23 & \cellcolor{brightlavender}-33.98 & \cellcolor{pink}-5.20 & \cellcolor{lightgreen}-0.85 \\ 
 & \textsc{Turkish} & 67.45 & \cellcolor{brightlavender}-46.69 & \cellcolor{lightgreen}-4.91 & \cellcolor{lightgreen}-2.61 & \cellcolor{brightlavender}-15.25 & \cellcolor{brightlavender}-10.34 & \cellcolor{brightlavender}-28.07 & \cellcolor{pink}-6.01 & \cellcolor{lightgreen}-0.83 \\ 
 & \textsc{Indonesian} & 54.10 & \cellcolor{brightlavender}-32.90 & \cellcolor{lightgreen}-4.91 & \cellcolor{lightgreen}-4.83 & \cellcolor{pink}-7.60 & \cellcolor{pink}-7.23 & \cellcolor{brightlavender}-17.99 & \cellcolor{pink}-8.04 & \cellcolor{pink}-5.87 \\ 
 & \textsc{Russian} & 58.28 & \cellcolor{brightlavender}-50.84 & \cellcolor{lightgreen}-2.65 & \cellcolor{lightgreen}-0.20 & \cellcolor{pink}-7.61 & \cellcolor{pink}-5.39 & \cellcolor{brightlavender}-23.62 & \cellcolor{pink}-6.25 & \cellcolor{mediumspringgreen}0.84 \\ 
 & \textsc{Arabic} & 41.88 & \cellcolor{brightlavender}-36.40 & \cellcolor{pink}-6.09 & \cellcolor{pink}-7.08 & \cellcolor{pink}-9.51 & \cellcolor{pink}-9.57 & \cellcolor{brightlavender}-20.03 & \cellcolor{lightgreen}-3.21 & \cellcolor{lightgreen}-0.65 \\ 
\hdashline 
Summary & \gap  & -20.53 & \cellcolor{brightlavender}-38.37 & \cellcolor{lightgreen}-22.74 & \cellcolor{lightgreen}-22.01 & \cellcolor{pink}-26.65 & \cellcolor{pink}-23.89 & \cellcolor{brightlavender}-30.72 & \cellcolor{lightgreen}-22.83 & \cellcolor{lightgreen}-21.20 
\\
\bottomrule

\end{tabular}
}
\caption{Relative Zero shot Cross-Lingual performance compared to reference (\textsc{Ref} column) when fine-tuning the model applying  \reinit (section \ref{sec:controlled_exp}) to specific set of layers. Source language is English. Bottom-line model \textsc{ALL} (for all layers randomly initialized) corresponds to a model trained from scratch on the task.
\textsc{Ref} column is the \standardFineTune fine-tuned model. 
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Std min/median/max,Parsing:0.02/0.34/1.48,POS:0.01/0.5/2.38 ,NER:0.0/0.47/2.62%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
}
\label{tab:re_init_x4_all_reduce}%re_init_x4_all_reduce}
\end{table*}

==> tables/re_init_x3_gap.tex <==




\begin{table*}[t!]
\footnotesize\centering
\scalebox{0.85}{ % was .7775
\begin{tabular}{llrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     &&&  \multicolumn{5}{c}{\textit{\reinit \textit{of layers}}} \\
     \cmidrule{4-8}
     Setting&Evaluation&\textsc{\standardFineTune} & \textsc{All} &  \textsc{0-2} & \textsc{3-5} & \textsc{6-8} &
     \textsc{9-11} &
    
    \midrule
    &&  \multicolumn{6}{c}{\textit{Parsing}} \\
    
  \textit{\inlang performance}& \textsc{English} & \textit{88.59} & \textit{74.58} & \textit{83.37} & \textit{85.54} & \textit{87.36} & \textit{88.62} \\ 
  \hdashline
 \gap& \textsc{French} & 19.65 & \cellcolor{brightlavender}70.88 & \cellcolor{brightlavender}39.56 & \cellcolor{lightgreen}23.77 & \cellcolor{lightgreen}20.34 & \cellcolor{mediumspringgreen}19.26 \\ 
 & \textsc{German} & 21.16 & \cellcolor{brightlavender}69.85 & \cellcolor{brightlavender}35.52 & \cellcolor{pink}26.61 & \cellcolor{lightgreen}23.24 & \cellcolor{lightgreen}21.95 \\ 
 & \textsc{Turkish} & 60.19 & \cellcolor{brightlavender}71.82 & \cellcolor{brightlavender}72.68 & \cellcolor{pink}65.31 & \cellcolor{lightgreen}61.97 & \cellcolor{mediumspringgreen}58.19 \\ 
 & \textsc{Indonesian} & 43.46 & \cellcolor{brightlavender}69.59 & \cellcolor{pink}50.30 & \cellcolor{lightgreen}44.89 & \cellcolor{mediumspringgreen}42.94 & \cellcolor{mediumspringgreen}41.66 \\ 
 & \textsc{Russian} & 28.89 & \cellcolor{brightlavender}71.63 & \cellcolor{pink}36.36 & \cellcolor{lightgreen}33.17 & \cellcolor{lightgreen}30.92 & \cellcolor{mediumspringgreen}27.21 \\ 
 & \textsc{Arabic} & 65.22 & \cellcolor{pink}71.39 & \cellcolor{lightgreen}67.20 & \cellcolor{lightgreen}66.70 & \cellcolor{lightgreen}66.66 & \cellcolor{mediumspringgreen}64.09 \\
\hdashline  
 & \textsc{Average }  & 39.76 & \cellcolor{brightlavender}70.86 & \cellcolor{brightlavender}50.27 & \cellcolor{lightgreen}43.41 & \cellcolor{lightgreen}41.01 &\cellcolor{lightgreen} 38.73 \\ 

\midrule
 &&  \multicolumn{6}{c}{\textit{POS}} \\
   \textit{\standardFineTune performance}& \textsc{English} & \textit{96.53} & \textit{87.71} & \textit{95.40} & \textit{95.59} & \textit{96.34} & \textit{96.74} \\ 
\hdashline    
 \gap& \textsc{French} & 8.28 & \cellcolor{brightlavender}58.75 & \cellcolor{brightlavender}25.98 & \cellcolor{lightgreen}9.18 & \cellcolor{lightgreen}9.40 & \cellcolor{lightgreen}8.45 \\ 
 & \textsc{German} & 5.89 & \cellcolor{brightlavender}58.78 & \cellcolor{brightlavender}23.77 & \cellcolor{lightgreen}7.30 & \cellcolor{lightgreen}6.09 & \cellcolor{lightgreen}5.91 \\ 
 & \textsc{Turkish} & 23.88 & \cellcolor{brightlavender}55.48 & \cellcolor{brightlavender}47.64 & \cellcolor{pink}29.23 & \cellcolor{lightgreen}25.43 & \cellcolor{mediumspringgreen}23.82 \\ 
 & \textsc{Indonesian} & 12.46 & \cellcolor{brightlavender}50.73 & \cellcolor{pink}19.47 & \cellcolor{lightgreen}13.61 & \cellcolor{lightgreen}12.56 & \cellcolor{mediumspringgreen}12.32 \\ 
 & \textsc{Russian} & 13.55 & \cellcolor{brightlavender}55.08 & \cellcolor{lightgreen}17.47 & \cellcolor{lightgreen}13.90 & \cellcolor{mediumspringgreen}13.36 & \cellcolor{lightgreen}14.99 \\ 
 & \textsc{Arabic} & 39.87 & \cellcolor{brightlavender}68.09 & \cellcolor{mediumspringgreen}37.48 & \cellcolor{lightgreen}40.90 & \cellcolor{lightgreen}40.30 & \cellcolor{lightgreen}40.77 \\ 
\hdashline 
 & \textsc{Average }  & 17.32 & \cellcolor{brightlavender}57.82 &\cellcolor{brightlavender} 28.63 & \cellcolor{lightgreen}19.02 & \cellcolor{lightgreen}17.86 & \cellcolor{lightgreen}17.71 \\ 
\midrule

 &&  \multicolumn{6}{c}{\textit{NER}} \\
  \textit{\inlang performance}   & \textsc{English} & \textit{83.06} & \textit{56.56} &\textit{76.68} & \textit{78.93} & \textit{81.64} & \textit{82.39} \\ 
\hdashline      
 \gap& \textsc{French} & 6.30 & \cellcolor{brightlavender}21.21 & \cellcolor{pink}11.54 & \cellcolor{lightgreen}8.59 & \cellcolor{mediumspringgreen}6.22 & \cellcolor{lightgreen}6.49 \\ 
 & \textsc{German} & 6.38 & \cellcolor{brightlavender}37.61 & \cellcolor{brightlavender}20.18 & \cellcolor{lightgreen}9.40 & \cellcolor{mediumspringgreen}6.26 & \cellcolor{mediumspringgreen}5.28 \\ 
 & \textsc{Turkish} & 15.42 & \cellcolor{brightlavender}35.80 & \cellcolor{pink}23.65 & \cellcolor{lightgreen}18.34 & \cellcolor{lightgreen}15.98 & \cellcolor{lightgreen}17.52 \\ 
 & \textsc{Indo} & 29.59 & \cellcolor{pink}35.36 & \cellcolor{lightgreen}32.93 & \cellcolor{lightgreen}31.10 & \cellcolor{mediumspringgreen}27.25 & \cellcolor{lightgreen}33.68 \\ 
 & \textsc{Russian} & 24.83 & \cellcolor{brightlavender}49.13 & \cellcolor{pink}33.85 & \cellcolor{pink}32.80 & \cellcolor{lightgreen}28.26 & \cellcolor{mediumspringgreen}24.30 \\ 
 & \textsc{Arabic} & 41.25 & \cellcolor{pink}51.08 & \cellcolor{pink}50.47 & \cellcolor{mediumspringgreen}40.05 & \cellcolor{lightgreen}43.09 & \cellcolor{mediumspringgreen}41.56 \\ 
\hdashline  
 & \textsc{Average }  & 20.63 & \cellcolor{brightlavender}38.37 & \cellcolor{pink}28.77 & \cellcolor{lightgreen}23.38 & \cellcolor{lightgreen}21.18 & \cellcolor{lightgreen}21.47 \\
\bottomrule

\end{tabular}
}
\caption{Zero-shot \gap between English (source) and the target languages when applying \reinit in comparison with the \standardFineTune fine-tuned model. The \gap is computed using English \textit{scores} as the reference.  % compared to the \standardFineTune fine-tuned model (\textsc{None}) when  applying \reinit %(section \ref{sec:controlled_exp})
%to specific layers. 
Baseline (\textsc{All}  layers randomly-initialized) corresponds to a model trained from scratch on the task.
%\textsc{Ref} column is the \standardFineTune fine-tuned model. 
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Each score is the mean over 5 random seed runs.  %{\small 
Std min/median/max,Parsing:0.02/0.34/1.48, POS:0.01/0.5/2.38, NER:0.0/0.47/2.62
%\colorbox{blue}{xxx}
\colorbox{mediumspringgreen}{$\leq$ \standardFineTune}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
\colorbox{lightgreen}{$>$ \standardFineTune}
\colorbox{pink}{$\geq$ +5 points}
\colorbox{brightlavender}{$\geq$ +10 points } }
%\textcolor{brightlavender}{$\leq$ 20 points drop}}
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
%}
\label{tab:re_init_x4_all_reduce}%re_init_x4_all_reduce}
\end{table*}

==> tables/re_init_x3_real.tex <==




\begin{table*}[t!]
\footnotesize\centering
\scalebox{0.85}{ % was .7775
\begin{tabular}{llrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     &&  \multicolumn{5}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     Setting&Evaluation&\textsc{\standardFineTune} & \Delta~\textsc{All} &  \Delta~\textsc{0-2} & \Delta~\textsc{3-5} & \Delta~\textsc{6-8} &
     \Delta~\textsc{9-11} &
    
    \midrule
    &&  \multicolumn{4}{c}{\textit{Parsing}} \\
     \inlang& \textsc{English} & 88.59 & \cellcolor{brightlavender}-14.01 & \cellcolor{pink}-5.22 & \cellcolor{lightgreen}-3.05 & \cellcolor{lightgreen}-1.23 & \cellcolor{mediumspringgreen}0.03 \\
\hdashline
 \crosslang& \textsc{French} & 68.94 & \cellcolor{brightlavender}-65.24 & \cellcolor{brightlavender}-25.13 & \cellcolor{pink}-7.17 & \cellcolor{lightgreen}-1.91 & \cellcolor{mediumspringgreen}0.42 \\ 
 & \textsc{German} & 67.43 & \cellcolor{brightlavender}-62.71 & \cellcolor{brightlavender}-19.59 & \cellcolor{pink}-8.50 & \cellcolor{lightgreen}-3.31 & \cellcolor{lightgreen}-0.77 \\ 
 & \textsc{Turkish} & 28.40 & \cellcolor{brightlavender}-25.65 & \cellcolor{brightlavender}-17.72 & \cellcolor{pink}-8.17 & \cellcolor{lightgreen}-3.01 & \cellcolor{mediumspringgreen}2.03 \\ 
 & \textsc{Indonesian} & 45.13 & \cellcolor{brightlavender}-40.14 & \cellcolor{brightlavender}-12.06 & \cellcolor{lightgreen}-4.48 & \cellcolor{lightgreen}-0.71 & \cellcolor{mediumspringgreen}1.83 \\ 
 & \textsc{Russian} & 59.70 & \cellcolor{brightlavender}-56.75 & \cellcolor{brightlavender}-12.69 & \cellcolor{pink}-7.32 & \cellcolor{lightgreen}-3.25 & \cellcolor{mediumspringgreen}1.71 \\ 
 & \textsc{Arabic} & 23.37 & \cellcolor{brightlavender}-20.18 & \cellcolor{pink}-7.21 & \cellcolor{lightgreen}-4.54 & \cellcolor{lightgreen}-2.67 & \cellcolor{mediumspringgreen}1.16 \\ 
%\hdashline
%&  Average  & 54.51 & \cellcolor{brightlavender}-40.67 & \cellcolor{pink}-14.23 & \cellcolor{pink}-6.18 & \cellcolor{mediumspringgreen}-2.30 & \cellcolor{green}+0.92 \\
\hdashline
%\midrule
 Summary & \gap  & -39.76 & -70.86 & -50.27 & -43.41 & -41.01 & -38.73 \\ 
\midrule
&&  \multicolumn{4}{c}{\textit{POS}} \\
 \inlang& \textsc{English} & 96.53 & \cellcolor{pink}-8.82 & \cellcolor{lightgreen}-1.12 & \cellcolor{lightgreen}-0.93 & \cellcolor{lightgreen}-0.18 & \cellcolor{mediumspringgreen}0.21 \\ 
 
 \hdashline
 \crosslang& \textsc{French} & 88.25 & \cellcolor{brightlavender}-59.29 & \cellcolor{brightlavender}-18.83 & \cellcolor{lightgreen}-1.83 & \cellcolor{lightgreen}-1.31 & \cellcolor{mediumspringgreen}0.04 \\ 
 & \textsc{German} & 90.63 & \cellcolor{brightlavender}-61.71 & \cellcolor{brightlavender}-19.00 & \cellcolor{lightgreen}-2.34 & \cellcolor{lightgreen}-0.38 & \cellcolor{mediumspringgreen}0.19 \\ 
 & \textsc{Turkish} & 72.65 & \cellcolor{brightlavender}-40.41 & \cellcolor{brightlavender}-24.88 & \cellcolor{pink}-6.28 & \cellcolor{lightgreen}-1.73 & \cellcolor{mediumspringgreen}0.27 \\ 
 & \textsc{Indonesian} & 84.06 & \cellcolor{brightlavender}-47.09 & \cellcolor{pink}-8.13 & \cellcolor{lightgreen}-2.08 & \cellcolor{lightgreen}-0.28 & \cellcolor{mediumspringgreen}0.35 \\ 
 & \textsc{Russian} & 82.97 & \cellcolor{brightlavender}-50.35 & \cellcolor{pink}-5.04 & \cellcolor{lightgreen}-1.28 & \cellcolor{mediumspringgreen}0.01 & \cellcolor{lightgreen}-1.22 \\ 
 & \textsc{Arabic} & 56.66 & \cellcolor{brightlavender}-37.05 & \cellcolor{mediumspringgreen}1.26 & \cellcolor{lightgreen}-1.97 & \cellcolor{lightgreen}-0.62 & \cellcolor{lightgreen}-0.69 \\ 
%& Avg  & 81.68 & 43.53 & 10.82 & 2.39 & 0.64 & 0.12 \\ 
\hdashline
Summary & \gap & -17.32 & -57.82 & -28.63 & -19.02 & -17.86 & -17.71 \\     

\midrule    
&&  \multicolumn{4}{c}{\textit{NER}} \\
 \inlang& \textsc{English} & 83.06 & \cellcolor{brightlavender}-26.50 & \cellcolor{pink}-6.38 & \cellcolor{lightgreen}-4.13 & \cellcolor{lightgreen}-1.42 & \cellcolor{lightgreen}-0.67 \\ 
 \crosslang& \textsc{French} & 76.76 & \cellcolor{brightlavender}-41.41 & \cellcolor{brightlavender}-11.62 & \cellcolor{pink}-6.42 & \cellcolor{lightgreen}-1.34 & \cellcolor{lightgreen}-0.86 \\ 
 & \textsc{German} & 76.68 & \cellcolor{brightlavender}-57.73 & \cellcolor{brightlavender}-20.18 & \cellcolor{pink}-7.15 & \cellcolor{lightgreen}-1.30 & \cellcolor{mediumspringgreen}0.43 \\ 
 & \textsc{Turkish} & 67.64 & \cellcolor{brightlavender}-46.88 & \cellcolor{brightlavender}-14.61 & \cellcolor{pink}-7.05 & \cellcolor{lightgreen}-1.98 & \cellcolor{lightgreen}-2.77 \\ 
 & \textsc{Indo} & 53.47 & \cellcolor{brightlavender}-32.27 & \cellcolor{pink}-9.72 & \cellcolor{pink}-5.64 & \cellcolor{mediumspringgreen}0.92 & \cellcolor{lightgreen}-4.76 \\ 
 & \textsc{Russian} & 58.23 & \cellcolor{brightlavender}-50.80 & \cellcolor{brightlavender}-15.40 & \cellcolor{brightlavender}-12.10 & \cellcolor{lightgreen}-4.85 & \cellcolor{lightgreen}-0.14 \\ 
 & \textsc{Arabic} & 41.81 & \cellcolor{brightlavender}-36.33 & \cellcolor{brightlavender}-15.60 & \cellcolor{lightgreen}-2.93 & \cellcolor{lightgreen}-3.26 & \cellcolor{lightgreen}-0.98 \\ 
%& Avg  & 65.38 & 41.70 & 13.36 & 6.49 & 1.89 & 1.39 \\ 
\hdashline
Summary & \gap  & -20.63 & -38.37 & -28.77 & -23.38 & -21.18 & -21.47 \\ 

\bottomrule

\end{tabular}
}
\caption{Zero-shot Cross-Lingual scores compared to the \standardFineTune fine-tuned model when  applying \reinit %(section \ref{sec:controlled_exp})
to specific layers. Source is English. Baseline (\textsc{All}  layers randomly-initialized) corresponds to a model trained from scratch on the task.
%\textsc{Ref} column is the \standardFineTune fine-tuned model. 
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Score mean of 5 random seed runs. {\small Std min/median/max,Parsing:0.02/0.34/1.48, POS:0.01/0.5/2.38, NER:0.0/0.47/2.62
%\colorbox{blue}{xxx}
\colorbox{mediumspringgreen}{$\geq$ reference}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
\colorbox{lightgreen}{$\leq$ reference}
\colorbox{pink}{$\geq$ 5 points drop}
\colorbox{brightlavender}{$\geq$ 15 points drop} }
%\textcolor{brightlavender}{$\leq$ 20 points drop}}
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
}
\label{tab:re_init_x4_all_reduce}%re_init_x4_all_reduce}
\end{table*}

==> tables/reinit_2x_layers_absolute.tex <==


\begin{table*}[h!]
\footnotesize\centering
\scalebox{0.78}{ % was .7775
\begin{tabular}{llrrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     && & \multicolumn{7}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     
     Setting&Eval&\textsc{\standardFineTune} & \textsc{All} & \textsc{0-1} & \textsc{2-3} & \textsc{4-5} & \textsc{6-7} &  \textsc{8-9} &  \textsc{10-11} \\
     &&\multicolumn{8}{c}{\textit{Parsing}}\\
     &\textsc{English} & 88.48 &\cellcolor{brightlavender}74.22& \cellcolor{lightgreen}87.71 & \cellcolor{lightgreen}87.34 & \cellcolor{lightgreen}87.04 & \cellcolor{lightgreen}87.67 & \cellcolor{lightgreen}88.24 & \cellcolor{mediumspringgreen}88.54 \\ 
&\textsc{French} & 66.95& \cellcolor{brightlavender}15.66& \cellcolor{brightlavender}50.21 & \cellcolor{pink}58.37 & \cellcolor{lightgreen}61.98 & \cellcolor{lightgreen}65.95 & \cellcolor{mediumspringgreen}67.21 & \cellcolor{mediumspringgreen}67.12 \\ 
&\textsc{German} & 64.83&\cellcolor{brightlavender}19.22 & \cellcolor{brightlavender}50.27 & \cellcolor{pink}56.24 & \cellcolor{lightgreen}59.56 & \cellcolor{lightgreen}62.66 & \cellcolor{mediumspringgreen}65.04 & \cellcolor{lightgreen}64.88 \\ 
&\textsc{Turkish} & 24.10&\cellcolor{brightlavender}7.28 & \cellcolor{brightlavender}12.79 & \cellcolor{pink}17.41 & \cellcolor{lightgreen}20.59 & \cellcolor{lightgreen}21.85 & \cellcolor{mediumspringgreen}25.36 & \cellcolor{lightgreen}23.87 \\ 
&\textsc{Indonesian} & 43.00 &\cellcolor{brightlavender}21.50& \cellcolor{pink}36.44 & \cellcolor{lightgreen}37.72 & \cellcolor{lightgreen}39.52 & \cellcolor{mediumspringgreen}43.09 & \cellcolor{mediumspringgreen}44.43 & \cellcolor{mediumspringgreen}43.39 \\ 
&\textsc{Russian} & 58.96 &\cellcolor{brightlavender}21.90& \cellcolor{pink}50.91 & \cellcolor{pink}52.49 & \cellcolor{lightgreen}53.33 & \cellcolor{lightgreen}55.88 & \cellcolor{lightgreen}58.13 & \cellcolor{lightgreen}58.57 \\ 
&\textsc{Arabic} & 22.91&\cellcolor{brightlavender}8.09 & \cellcolor{lightgreen}21.55 & \cellcolor{lightgreen}18.75 & \cellcolor{lightgreen}18.33 & \cellcolor{lightgreen}20.63 & \cellcolor{lightgreen}22.02 & \cellcolor{lightgreen}20.85 \\ 
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    \midrule

\bottomrule

\end{tabular}
}
\caption{Absolute Zero shot Cross-Lingual performance compared to reference (\textsc{Ref} column) when fine-tuning the model applying  \reinit (section \ref{sec:controlled_exp}) to specific set of layers. Source language is English. Baseline \textsc{ALL} (for all layers randomly initialized) corresponds to a model trained from scratch on the task.
\textsc{Ref} column is model \standardFineTune fine-tuned model. 
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Std min/median/max NER:0.0/0.47/2.62
\bm{add std for all}
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
}
\label{tab:absolute_re_init_x2}%re_init_x4_all_reduce}
\end{table*}

==> tables/reinit_word_pos.tex <==


\begin{table}[h!]
\footnotesize\centering
\scalebox{0.75}{ % was .7775
\begin{tabular}{lrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     &\textsc{Ref} & \textsc{Word} & \textsc{Pos} \\
     %\textit{Re-Init.} & \textsc{None } & \textsc{0} & \textsc{1} & \textsc{2} & \textsc{5} & \textsc{8} & \textsc{10} & \textsc{11} & \textsc{0-1} & \textsc{1-2} & \textsc{2-3} & \textsc{4-5} & \textsc{6-7} & \textsc{8-9} & \textsc{10-11} & \textsc{0-2} & \textsc{1-3} & \textsc{4-6} & \textsc{9-11}  \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    \midrule
&\multicolumn{3}{c}{\textit{Parsing}}\\
\textsc{Eng} & 89.06 & \cellcolor{pink}70.47 & \cellcolor{pink}85.76 \\
\textsc{Fre} & 69.92 & \cellcolor{brightlavender}3.09 & \cellcolor{pink}61.60\\
\textsc{Ger} & 67.62 & \cellcolor{brightlavender}4.43 & \cellcolor{pink}62.80 \\
\textsc{Tur} & 30.06 & \cellcolor{brightlavender}2.97 & \cellcolor{pink}22.87 \\
\textsc{Ind} & 47.58 & \cellcolor{brightlavender}4.33 & \cellcolor{pink}42.18 \\
\textsc{Rus} & 60.67 & \cellcolor{brightlavender}3.20 & \cellcolor{pink}50.89 \\
\textsc{Ara} & 26.59 & \cellcolor{brightlavender}1.37 & \cellcolor{pink}14.27 & \\
 
\midrule
&\multicolumn{3}{c}{\textit{POS}}\\

\textsc{Eng} & 96.19 & \cellcolor{pink}89.83 & \cellcolor{pink}93.64 \\ 
\textsc{Fre} & 88.58 & \cellcolor{brightlavender}27.92 & \cellcolor{pink}83.71 \\
\textsc{Ger} & 89.36 & \cellcolor{brightlavender}30.34 & \cellcolor{pink}85.49  \\ 
\textsc{Tur} & 73.30 & \cellcolor{brightlavender}33.26 & \cellcolor{pink}61.97   \\ 
\textsc{Ind} & 83.94 & \cellcolor{brightlavender}36.53 & \cellcolor{lightgreen}82.01 \\ 
\textsc{Rus} & 81.89 & \cellcolor{brightlavender}33.59 & \cellcolor{pink}75.53  \\ 
\textsc{Ara} & 56.68 & \cellcolor{brightlavender}18.05 & \cellcolor{pink}49.09 & \\
\midrule
&\multicolumn{3}{c}{\textit{NER}}\\

\textsc{Eng} & 83.08 & \cellcolor{brightlavender}46.77 & \cellcolor{pink}69.25 \\

\textsc{Fre} & 78.57 & \cellcolor{brightlavender}25.02 & \cellcolor{pink}65.86  \\ 
\textsc{Ger} & 78.53 & \cellcolor{brightlavender}18.90 & \cellcolor{pink}59.66  \\ 

\textsc{Tur} & 72.81 & \cellcolor{brightlavender}19.38 & \cellcolor{pink}56.04  \\ 

\textsc{Ind} & 57.16 & \cellcolor{brightlavender}19.11 & \cellcolor{pink}47.85   \\

\textsc{Rus} & 63.64 & \cellcolor{brightlavender}6.84 & \cellcolor{brightlavender}43.14 \\ 
\textsc{Ara} & 43.25 & \cellcolor{brightlavender}7.05 & \cellcolor{pink}29.11  \\

\bottomrule



\end{tabular}
}
\caption{Absolute Zero shot Cross-Lingual performance compapink to reference (\textsc{Ref} column) when fine-tuning the model applying  \reinit to layers \textsc{Word/Position} Embedding (\textsc{Word/Pos}), Reference column is model fine-tuned when no \reinit is applied. 
\\
%\textit{In-Lang} and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer
%\colorbox{blue!30}{okkk}
%\textcolor{green}{$\geq$ reference}
~~ \colorbox{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
\colorbox{pink}{$\geq$ 3 points drop} ~~
\colorbox{brightlavender}{$\geq$ 20 points drop}}
%Drop in performance highlighted in pink \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
\label{tab:re_init_x1_x2_x3_absolute_appendix}
\end{table}

==> tables/reinit_x2_delta_regroup.tex <==


\begin{table}[t!]
\footnotesize\centering
\scalebox{0.7}{ % was .7775
\begin{tabular}{lrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
      & \multicolumn{7}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     \textsc{Src-Trg}&\textsc{\standardFineTune} & \Delta \textsc{1-2} & \Delta \textsc{3-4} & \Delta \textsc{5-6} & \Delta \textsc{7-8} & \Delta \textsc{9-10} &  \Delta \textsc{11-12} \\
     &\multicolumn{7}{c}{\textit{Parsing}}\\
 \textsc{EN-EN} & 88.48 & \cellcolor{lightgreen}-0.77 & \cellcolor{lightgreen}-1.14 & \cellcolor{lightgreen}-1.44 & \cellcolor{lightgreen}-0.81 & \cellcolor{lightgreen}-0.24 & \cellcolor{mediumspringgreen}0.06 \\ 
 \textsc{RU-RU} & 87.31 & \cellcolor{mediumspringgreen}0.19 & \cellcolor{lightgreen}-0.94 & \cellcolor{lightgreen}-0.61 & \cellcolor{mediumspringgreen}0.27 & \cellcolor{mediumspringgreen}0.92 & \cellcolor{mediumspringgreen}0.97 \\ 
 \textsc{AR-AR} & 83.09 & \cellcolor{lightgreen}-0.95 & \cellcolor{lightgreen}-1.26 & \cellcolor{lightgreen}-1.17 & \cellcolor{lightgreen}-0.82 & \cellcolor{lightgreen}-0.18 & \cellcolor{mediumspringgreen}0.12 \\ 
 \hdashline 
 \textsc{EN-X }  &  52.75 & \cellcolor{brightlavender} -8.48 & \cellcolor{brightlavender} -5.84 & \cellcolor{pink} -4.12 & \cellcolor{lightgreen} -1.64 & \cellcolor{mediumspringgreen} 0.17 & \cellcolor{lightgreen} -0.29 \\ 
\textsc{RU-X}  &  55.81 & \cellcolor{brightlavender} -8.00 & \cellcolor{pink} -3.76 & \cellcolor{pink} -3.32 & \cellcolor{pink} -2.30 & \cellcolor{mediumspringgreen} 0.87 & \cellcolor{mediumspringgreen} 0.33 \\ 
\textsc{AR-X }  &  35.78 & \cellcolor{pink} -4.41 & \cellcolor{pink} -2.54 & \cellcolor{lightgreen} -2.00 & \cellcolor{lightgreen} -1.22 & \cellcolor{lightgreen} -0.76 & \cellcolor{mediumspringgreen} 0.16 \\ 

 \midrule
      &\multicolumn{7}{c}{\textit{POS}}\\
\textsc{EN-EN} & 96.46 & \cellcolor{lightgreen}-0.49 & \cellcolor{lightgreen}-0.42 & \cellcolor{lightgreen}-0.34 & \cellcolor{lightgreen}-0.08 & \cellcolor{mediumspringgreen}0.10 & \cellcolor{mediumspringgreen}0.12 \\ 
\textsc{RU-RU} & 98.08 & \cellcolor{lightgreen}-0.41 & \cellcolor{lightgreen}-0.52 & \cellcolor{lightgreen}-0.37 & \cellcolor{lightgreen}-0.13 & \cellcolor{mediumspringgreen}0.03 & \cellcolor{mediumspringgreen}0.01 \\ 
\textsc{AR-AR} & 96.46 & \cellcolor{lightgreen}-0.39 & \cellcolor{lightgreen}-0.44 & \cellcolor{lightgreen}-0.41 & \cellcolor{lightgreen}-0.14 & \cellcolor{mediumspringgreen}0.02 & \cellcolor{lightgreen}-0.02 \\ 
\hdashline
\textsc{EN-X}  &  81.11 & \cellcolor{brightlavender} -6.90 & \cellcolor{pink} -3.16 & \cellcolor{lightgreen} -1.65 & \cellcolor{lightgreen} -0.08 & \cellcolor{lightgreen} -0.32 & \cellcolor{mediumspringgreen} 0.02 \\ 
 

\textsc{RU-X}  &  80.46 & \cellcolor{brightlavender} -8.88 & \cellcolor{brightlavender} -5.09 & \cellcolor{pink} -3.27 & \cellcolor{lightgreen} -0.41 & \cellcolor{mediumspringgreen} 0.94 & \cellcolor{lightgreen} -0.36 \\ 
 

\textsc{AR-X }  &  68.22 & \cellcolor{brightlavender} -6.28 & \cellcolor{pink} -3.22 & \cellcolor{lightgreen} -0.98 & \cellcolor{lightgreen} -1.58 & \cellcolor{lightgreen} -0.82 & \cellcolor{lightgreen} -0.51 \\ 
 \midrule
 
 
&\multicolumn{7}{c}{\textit{NER}}\\
 \textsc{EN-EN} & 82.99 & \cellcolor{pink}-2.16 & \cellcolor{lightgreen}-1.95 & \cellcolor{lightgreen}-1.04 & \cellcolor{lightgreen}-0.16 & \cellcolor{mediumspringgreen}0.06 &
 \cellcolor{mediumspringgreen}0.16 \\ 
 \textsc{RU-RU} & 88.19 & \cellcolor{lightgreen}-1.92 & \cellcolor{pink}-2.04 & \cellcolor{lightgreen}-1.44 & \cellcolor{lightgreen}-0.57 & \cellcolor{lightgreen}-0.34 & \cellcolor{lightgreen}-0.07 \\ 
 \textsc{AR-AR} & 88.06 & \cellcolor{pink}-2.34 & \cellcolor{lightgreen}-1.97 & \cellcolor{lightgreen}-0.99 & \cellcolor{lightgreen}-0.45 & \cellcolor{lightgreen}-0.17 & \cellcolor{mediumspringgreen}0.07 \\ 
 \hdashline
\textsc{EN-X }  &  64.36 & \cellcolor{brightlavender} -5.97 & \cellcolor{pink} -4.26 & \cellcolor{pink} -2.32 & \cellcolor{lightgreen} -0.25 & \cellcolor{lightgreen} -0.02 & \cellcolor{mediumspringgreen} 0.43 \\ 
\textsc{RU-X}  & 61.24 & \cellcolor{brightlavender} -12.93 & \cellcolor{brightlavender} -8.88 & \cellcolor{pink} -4.57 & \cellcolor{pink} -2.93 & \cellcolor{pink} -2.27 & \cellcolor{lightgreen} -0.49 \\ 
\textsc{AR-X}  & 66.75 & \cellcolor{brightlavender} -12.10 & \cellcolor{brightlavender} -7.11 & \cellcolor{pink} -4.69 & \cellcolor{lightgreen} -1.39 & \cellcolor{lightgreen} -1.05 & \cellcolor{mediumspringgreen} 0.21 \\
 
\bottomrule

\end{tabular}
}

\caption{Relative Zero shot Cross-Lingual performance compared to \standardFineTune fine-tuned models when applying  \reinit (section \ref{sec:controlled_exp}) to pairs of consecutive  layers. NB: \textsc{Lang-Lang} stands for \inlang performance for the given \textsc{Lang}. \textsc{Lang-X} refers to \crosslang performance with \textsc{Lang} as the source language averaged over all the target languages.  
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
%Std min/median/max NER:0.0/0.47/2.62
\colorbox{mediumspringgreen}{$\geq$ \textsc{\standardFineTune}}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
\colorbox{lightgreen}{$<$  \textsc{\standardFineTune}}
\colorbox{pink}{$\leq$ -2 points}
\colorbox{brightlavender}{$\leq$ -5 points }
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
}
\label{tab:delta_standard_re_init_x2}%re_init_x4_all_reduce}
\end{table}

==> tables/reinit_x2_deta.tex <==


\begin{table*}[h!]
\footnotesize\centering
\scalebox{0.78}{ % was .7775
\begin{tabular}{llrrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
       & & \multicolumn{8}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     Setting&Eval&\textsc{\standardFineTune} & \Delta \textsc{All} & \Delta \textsc{0-1} & \Delta \textsc{2-3} & \Delta \textsc{4-5} & \Delta \textsc{6-7} & \Delta \textsc{8-9} &  \Delta \textsc{10-11} \\
     &&\multicolumn{8}{c}{\textit{Parsing}}\\
 \textit{\inlang}&\textsc{English} & 88.48 && \cellcolor{lightgreen}-0.77 & \cellcolor{lightgreen}-1.14 & \cellcolor{lightgreen}-1.44 & \cellcolor{lightgreen}-0.81 & \cellcolor{lightgreen}-0.24 & \cellcolor{mediumspringgreen}0.06 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  &  52.75 && \cellcolor{brightlavender} -8.48 & \cellcolor{brightlavender} -5.84 & \cellcolor{pink} -4.12 & \cellcolor{lightgreen} -1.64 & \cellcolor{mediumspringgreen} 0.17 & \cellcolor{lightgreen} -0.29 \\ 

 \hdashline 
 \textit{\inlang}&\textsc{Russian} & 87.31 && \cellcolor{mediumspringgreen}0.19 & \cellcolor{lightgreen}-0.94 & \cellcolor{lightgreen}-0.61 & \cellcolor{mediumspringgreen}0.27 & \cellcolor{mediumspringgreen}0.92 & \cellcolor{mediumspringgreen}0.97 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  &  55.81 && \cellcolor{brightlavender} -8.00 & \cellcolor{pink} -3.76 & \cellcolor{pink} -3.32 & \cellcolor{pink} -2.30 & \cellcolor{mediumspringgreen} 0.87 & \cellcolor{mediumspringgreen} 0.33 \\ 
 \hdashline 
\textit{\inlang}&\textsc{Arabic} & 83.09 && \cellcolor{lightgreen}-0.95 & \cellcolor{lightgreen}-1.26 & \cellcolor{lightgreen}-1.17 & \cellcolor{lightgreen}-0.82 & \cellcolor{lightgreen}-0.18 & \cellcolor{mediumspringgreen}0.12 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  &  35.78 && \cellcolor{pink} -4.41 & \cellcolor{pink} -2.54 & \cellcolor{lightgreen} -2.00 & \cellcolor{lightgreen} -1.22 & \cellcolor{lightgreen} -0.76 & \cellcolor{mediumspringgreen} 0.16 \\ 
 \midrule
      &&\multicolumn{8}{c}{\textit{POS}}\\

\textit{\inlang}&\textsc{English} & 96.46 && \cellcolor{lightgreen}-0.49 & \cellcolor{lightgreen}-0.42 & \cellcolor{lightgreen}-0.34 & \cellcolor{lightgreen}-0.08 & \cellcolor{mediumspringgreen}0.10 & \cellcolor{mediumspringgreen}0.12 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  &  81.11 && \cellcolor{brightlavender} -6.90 & \cellcolor{pink} -3.16 & \cellcolor{lightgreen} -1.65 & \cellcolor{lightgreen} -0.08 & \cellcolor{lightgreen} -0.32 & \cellcolor{mediumspringgreen} 0.02 \\ 
 \hdashline 
\textit{\inlang}&\textsc{Russian} & 98.08 && \cellcolor{lightgreen}-0.41 & \cellcolor{lightgreen}-0.52 & \cellcolor{lightgreen}-0.37 & \cellcolor{lightgreen}-0.13 & \cellcolor{mediumspringgreen}0.03 & \cellcolor{mediumspringgreen}0.01 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  &  80.46 && \cellcolor{brightlavender} -8.88 & \cellcolor{brightlavender} -5.09 & \cellcolor{pink} -3.27 & \cellcolor{lightgreen} -0.41 & \cellcolor{mediumspringgreen} 0.94 & \cellcolor{lightgreen} -0.36 \\ 
 \hdashline 
\textit{\inlang}&\textsc{Arabic} & 96.46 && \cellcolor{lightgreen}-0.39 & \cellcolor{lightgreen}-0.44 & \cellcolor{lightgreen}-0.41 & \cellcolor{lightgreen}-0.14 & \cellcolor{mediumspringgreen}0.02 & \cellcolor{lightgreen}-0.02 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  &  68.22 && \cellcolor{brightlavender} -6.28 & \cellcolor{pink} -3.22 & \cellcolor{lightgreen} -0.98 & \cellcolor{lightgreen} -1.58 & \cellcolor{lightgreen} -0.82 & \cellcolor{lightgreen} -0.51 \\ 
 \midrule
&&\multicolumn{8}{c}{\textit{NER}}\\
 \textit{\inlang}&\textsc{English} & 82.99 && \cellcolor{pink}-2.16 & \cellcolor{lightgreen}-1.95 & \cellcolor{lightgreen}-1.04 & \cellcolor{lightgreen}-0.16 & \cellcolor{mediumspringgreen}0.06 & \cellcolor{mediumspringgreen}0.16 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  &  64.36 && \cellcolor{brightlavender} -5.97 & \cellcolor{pink} -4.26 & \cellcolor{pink} -2.32 & \cellcolor{lightgreen} -0.25 & \cellcolor{lightgreen} -0.02 & \cellcolor{mediumspringgreen} 0.43 \\ 
 \hdashline 
 \textit{\inlang}&\textsc{Russian} & 88.19 && \cellcolor{lightgreen}-1.92 & \cellcolor{pink}-2.04 & \cellcolor{lightgreen}-1.44 & \cellcolor{lightgreen}-0.57 & \cellcolor{lightgreen}-0.34 & \cellcolor{lightgreen}-0.07 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  & 61.24 && \cellcolor{brightlavender} -12.93 & \cellcolor{brightlavender} -8.88 & \cellcolor{pink} -4.57 & \cellcolor{pink} -2.93 & \cellcolor{pink} -2.27 & \cellcolor{lightgreen} -0.49 \\ 
 \hdashline 
 \textit{\inlang}&\textsc{Arabic} & 88.06 && \cellcolor{pink}-2.34 & \cellcolor{lightgreen}-1.97 & \cellcolor{lightgreen}-0.99 & \cellcolor{lightgreen}-0.45 & \cellcolor{lightgreen}-0.17 & \cellcolor{mediumspringgreen}0.07 \\ 
\textit{\crosslang} & \textsc{Mean Target Languages }  & 66.75 && \cellcolor{brightlavender} -12.10 & \cellcolor{brightlavender} -7.11 & \cellcolor{pink} -4.69 & \cellcolor{lightgreen} -1.39 & \cellcolor{lightgreen} -1.05 & \cellcolor{mediumspringgreen} 0.21 \\ 
 
 
 



    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    

\bottomrule

\end{tabular}
}
\caption{Relative Zero shot Cross-Lingual performance compared to \standardFineTune fine-tuned models when applying  \reinit (section \ref{sec:controlled_exp}) to pairs of consecutive  layers. Baseline \textsc{ALL} (for all layers randomly initialized) corresponds to a model trained from scratch on the task.
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Std min/median/max NER:0.0/0.47/2.62
\colorbox{mediumspringgreen}{$\geq$ \textsc{\standardFineTune}}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
\colorbox{lightgreen}{$<$  \textsc{\standardFineTune}}
\colorbox{pink}{$\leq$ -2 points}
\colorbox{brightlavender}{$\leq$ -5 points }
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
\bm{Would you have suggestions to better report these results ? }
}
\label{tab:absolute_re_init_x2}%re_init_x4_all_reduce}
\end{table*}

==> tables/reinit_x2_detla_english_source.tex <==


\begin{table*}[h!]
\footnotesize\centering
\scalebox{0.78}{ % was .7775
\begin{tabular}{llrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
       & & &\multicolumn{6}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     Setting&Eval&\textsc{\standardFineTune} & \Delta  \textsc{0-1} & \Delta \textsc{2-3} & \Delta \textsc{4-5} & \Delta \textsc{6-7} & \Delta \textsc{8-9} &  \Delta \textsc{10-11} \\
     &&\multicolumn{7}{c}{\textit{Parsing}}\\
 \textit{\inlang}&\textsc{English} & 88.52 & \cellcolor{lightgreen}-0.81 & \cellcolor{lightgreen}-1.18 & \cellcolor{lightgreen}-1.48 & \cellcolor{lightgreen}-0.85 & \cellcolor{lightgreen}-0.27 & \cellcolor{mediumspringgreen}0.02 \\ 
\textit{\crosslang}&\textsc{French} & 65.71 & \cellcolor{brightlavender}-15.50 & \cellcolor{brightlavender}-7.33 & \cellcolor{pink}-3.73 & \cellcolor{mediumspringgreen}0.25 & \cellcolor{mediumspringgreen}1.50 & \cellcolor{mediumspringgreen}1.41 \\ 
&\textsc{German} & 63.67 & \cellcolor{brightlavender}-13.41 & \cellcolor{brightlavender}-7.44 & \cellcolor{pink}-4.11 & \cellcolor{lightgreen}-1.02 & \cellcolor{mediumspringgreen}1.37 & \cellcolor{mediumspringgreen}1.20 \\ 
&\textsc{Turkish} & 22.92 & \cellcolor{brightlavender}-10.13 & \cellcolor{brightlavender}-5.51 & \cellcolor{pink}-2.34 & \cellcolor{lightgreen}-1.08 & \cellcolor{mediumspringgreen}2.44 & \cellcolor{mediumspringgreen}0.95 \\ 
&\textsc{Indonesian} & 42.18 & \cellcolor{brightlavender}-5.74 & \cellcolor{pink}-4.46 & \cellcolor{pink}-2.66 & \cellcolor{mediumspringgreen}0.91 & \cellcolor{mediumspringgreen}2.25 & \cellcolor{mediumspringgreen}1.21 \\ 
&\textsc{Russian} & 57.61 & \cellcolor{brightlavender}-6.69 & \cellcolor{brightlavender}-5.11 & \cellcolor{pink}-4.28 & \cellcolor{lightgreen}-1.73 & \cellcolor{mediumspringgreen}0.52 & \cellcolor{mediumspringgreen}0.96 \\ 
%&\textsc{Arabic} & 23.60 & \cellcolor{pink}-2.05 & \cellcolor{pink}-4.86 & \cellcolor{brightlavender}-5.27 & \cellcolor{pink}-2.98 & \cellcolor{lightgreen}-1.58 & \cellcolor{pink}-2.76 \\ 
%\textit{\crosslang} & \textsc{Mean Target Languages }  & \cellcolor{mediumspringgreen} 52.03 & \cellcolor{brightlavender} -7.76 & \cellcolor{brightlavender} -5.13 & \cellcolor{pink} -3.41 & \cellcolor{lightgreen} -0.93 & \cellcolor{mediumspringgreen} 0.89 & \cellcolor{mediumspringgreen} 0.43 \\ 
 


    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    

\bottomrule

\end{tabular}
}
\caption{Relative Zero shot Cross-Lingual performance compared to \standardFineTune fine-tuned models when applying  \reinit (section \ref{sec:controlled_exp}) to pairs of consecutive  layers. Baseline \textsc{ALL} (for all layers randomly initialized) corresponds to a model trained from scratch on the task.
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
Std min/median/max NER:0.0/0.47/2.62
\colorbox{mediumspringgreen}{$\geq$ \textsc{\standardFineTune}}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
\colorbox{lightgreen}{$<$  \textsc{\standardFineTune}}
\colorbox{pink}{$\leq$ -2 points}
\colorbox{brightlavender}{$\leq$ -5 points }
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
\bm{Would you have suggestions to better report these results ? }
}
\label{tab:absolute_re_init_x2}%re_init_x4_all_reduce}
\end{table*}

==> tables/reinit_x2_domain_delta.tex <==


\begin{table*}[h!]
\footnotesize\centering
\scalebox{0.78}{ % was .7775
\begin{tabular}{llrrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
       &&  \multicolumn{7}{c}{\underline{\textit{\reinit \textit{of layers}}}} \\
     Setting&\textsc{Source - Target}&\textsc{\standardFineTune}  & \Delta \textsc{0-1} & \Delta \textsc{2-3} & \Delta \textsc{4-5} & \Delta \textsc{6-7} & \Delta \textsc{8-9} &  \Delta \textsc{10-11} \\
     &&\multicolumn{7}{c}{\textit{Parsing}}\\
     
 \multicolumn{1}{c}{\textit{domain analyses}}&\textsc{En - En } & 90.40 & \cellcolor{lightgreen}-1.41 & \cellcolor{pink}-2.33 & \cellcolor{lightgreen}-1.57 & \cellcolor{lightgreen}-1.43 & \cellcolor{lightgreen}-0.60 & \cellcolor{lightgreen}-0.46 \\ 
&\textsc{En - En Literature} & 77.91 & \cellcolor{lightgreen}-0.91 & \cellcolor{lightgreen}-1.38 & \cellcolor{lightgreen}-1.85 & \cellcolor{lightgreen}-0.83 & \cellcolor{lightgreen}-0.23 & \cellcolor{lightgreen}-0.17 \\ 
&\textsc{En - En Web} & 75.77 & \cellcolor{pink}-2.14 & \cellcolor{pink}-2.42 & \cellcolor{pink}-2.54 & \cellcolor{lightgreen}-1.42 & \cellcolor{lightgreen}-0.71 & \cellcolor{lightgreen}-0.69 \\ 
&\textsc{En - En UGC} & 45.90 & \cellcolor{lightgreen}-1.97 & \cellcolor{pink}-2.75 & \cellcolor{pink}-2.10 & \cellcolor{lightgreen}-1.04 & \cellcolor{lightgreen}-0.39 & \cellcolor{lightgreen}-0.25 \\ 
\hdashline
\textit{\crosslang}&
\textsc{En - French translation} & 83.25 & \cellcolor{brightlavender}-5.82 & \cellcolor{pink}-2.69 & \cellcolor{pink}-2.42 & \cellcolor{lightgreen}-0.44 & \cellcolor{mediumspringgreen}0.25 & \cellcolor{mediumspringgreen}0.94 \\ 
&\textsc{En - French Wiki} & 71.29 & \cellcolor{brightlavender}-7.86 & \cellcolor{pink}-4.33 & \cellcolor{pink}-4.64 & \cellcolor{lightgreen}-0.92 & \cellcolor{lightgreen}-0.11 & \cellcolor{mediumspringgreen}0.33 \\ 
\midrule
     &&\multicolumn{7}{c}{\textit{POS}}\\
\textit{domain analyses}&\textsc{En - En} & 96.83 & \cellcolor{lightgreen}-1.35 & \cellcolor{lightgreen}-0.98 & \cellcolor{lightgreen}-0.70 & \cellcolor{lightgreen}-0.40 & \cellcolor{lightgreen}-0.28 & \cellcolor{lightgreen}-0.24 \\ 
&\textsc{En - En Litterature} & 93.09 & \cellcolor{lightgreen}-0.58 & \cellcolor{lightgreen}-0.65 & \cellcolor{lightgreen}-0.28 & \cellcolor{lightgreen}-0.04 & \cellcolor{lightgreen}-0.06 & \cellcolor{mediumspringgreen}0.12 \\ 
&\textsc{En - En Web} & 89.67 & \cellcolor{lightgreen}-1.07 & \cellcolor{lightgreen}-1.21 & \cellcolor{lightgreen}-0.41 & \cellcolor{lightgreen}-0.10 & \cellcolor{mediumspringgreen}0.03 & \cellcolor{mediumspringgreen}0.21 \\ 
&\textsc{En - En UGC} & 68.93 & \cellcolor{pink}-2.38 & \cellcolor{lightgreen}-1.07 & \cellcolor{lightgreen}-0.14 & \cellcolor{mediumspringgreen}0.54 & \cellcolor{lightgreen}-0.04 & \cellcolor{mediumspringgreen}0.63 \\ 
\hdashline
\textit{\crosslang}&
\textsc{En - French Translation} & 93.43 & \cellcolor{pink}-3.59 & \cellcolor{lightgreen}-0.88 & \cellcolor{lightgreen}-1.31 & \cellcolor{lightgreen}-0.56 & \cellcolor{mediumspringgreen}0.46 & \cellcolor{mediumspringgreen}0.25 \\ 
&\textsc{En - French} & 91.13 & \cellcolor{brightlavender}-5.10 & \cellcolor{lightgreen}-0.93 & \cellcolor{lightgreen}-1.16 & \cellcolor{lightgreen}-0.74 & \cellcolor{mediumspringgreen}0.15 & \cellcolor{lightgreen}-0.07 \\ 
\midrule
&&\multicolumn{7}{c}{\textit{NER}}\\
\textit{domain analyses}& \textsc{En - En} & 83.22 & \cellcolor{pink}-2.45 & \cellcolor{pink}-2.15 & \cellcolor{lightgreen}-1.28 & \cellcolor{lightgreen}-0.49 & \cellcolor{lightgreen}-0.15 & \cellcolor{lightgreen}-0.06 \\ 
&\textsc{En - News} & 51.72 & \cellcolor{lightgreen}-1.32 & \cellcolor{lightgreen}-1.05 & \cellcolor{lightgreen}-0.80 & \cellcolor{lightgreen}-0.14 & \cellcolor{lightgreen}-0.31 & \cellcolor{lightgreen}-0.33 \\ 
 \hdashline
 \multicolumn{1}{c}{\textit{\crosslang}}&\textsc{En - French} &76.16 & \cellcolor{brightlavender}-5.14 & \cellcolor{pink}-2.82 & \cellcolor{lightgreen}-1.97 & \cellcolor{lightgreen}-0.33 & \cellcolor{mediumspringgreen}0.52 & \cellcolor{mediumspringgreen}0.34 \\ 



    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
    

\bottomrule

\end{tabular}
}
\caption{
Relative Zero shot Cross-Lingual performance of \mbert with \reinit (section \ref{sec:controlled_exp}) on pairs of consecutive layers compared to \mbert without any random-initialization (\standardFineTune). We present experiments with English as the source language and evaluate across different target domains on English in comparison with the cross-lingual setting when we evaluate on French. 
%\inlang and \textit{Cross-Lang} comparison show that bottom layers are critical for \crosslang transfer while not for \inlang transfer. 
\colorbox{mediumspringgreen}{$\geq$ \textsc{\standardFineTune}}
%\textcolor{mediumspringgreen}{$\geq$ reference} ~~
\colorbox{lightgreen}{$<$  \textsc{\standardFineTune}}
\colorbox{pink}{$\leq$ -2 points}
\colorbox{brightlavender}{$\leq$ -5 points }
%\ye{is the avg row useful?}
%\\
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
% PARSING jobs 10521617 10541358
% POS jobs 10495788 att, 10560067 emb (standart)
% NER jobs  "10561501 reinit att 10560075 emb
%Drop in performance highlighted in red \cellcolor{pink} in cross-lingual setting : The syntactic cross-lingual transfer is localized in the two two first attention layer
%\ye{why did..}% you chose specifically these buckets? it might be the case for example that if you'd remove 4 layers at the end and 4 in the middle (instead of the current 3 and 5), they would look more similar. do we have this result to report and add to the appendix?}
}
\label{tab:re_init_x2_domain_delta}%re_init_x4_all_reduce}
\end{table*}

==> tables/top_vs_bottom.tex <==

\begin{table}[h!]
\footnotesize\centering
\scalebox{0.9}{ % was .7775
\begin{tabular}{lrr}
    \toprule
    %Scenario  & 
    \textit{Model} & \textsc{Bottom-3} & \textsc{Top-3} & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     %\textit{Fine-tuning} & \textsc{Standart} & \textsc{Attention only} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
&\multicolumn{2}{c}{\textit{Parsing}}\\

%\textsc{English} & 87.04 & 79.18 \\ \textsc{\crosslang Gap} & -40.62 & -57.83 \\ 
% reporting result ~ bottom-3 instead of bottom-5
\textsc{English} & 83.04 & 74.18 \\ %\textsc{\gap} & 40.62 & 57.83 \\
\textsc{\gap} & 40.62 & 67.81 \\ 

\midrule

&\multicolumn{2}{c}{\textit{POS}}\\
\textsc{English} & 94.06 & 90.95 \\
\gap & 17.74 & 34.96 \\ 
\midrule
&\multicolumn{2}{c}{\textit{NER}}\\
\textsc{English} & 73.09 & 65.71 \\ 

\gap & 20.47 & 31.48 \\ 


\bottomrule


\end{tabular}
}
\caption{
Cross-Lingual Gap averaged across all target languages for \textsc{Bottom-3}: model composed of  the 3 first layers, \textsc{Top-3}: model composed of the 3 last layers \\
}
\label{tab:top_vs_bottom_gap}
\end{table}
